Identifier Namespaces in Mathematical Notation

In this thesis, we look at the problem of assigning each identifier of a document to a namespace. At the moment, there does not exist a special dataset where all identifiers are grouped to namespaces, and therefore we need to create such a dataset ourselves. To do that, we need to find groups of documents that use identifiers in the same way. This can be done with cluster analysis methods. We argue that documents can be represented by the identifiers they contain, and this approach is similar to representing textual information in the Vector Space Model. Because of this, we can apply traditional document clustering techniques for namespace discovery. Because the problem is new, there is no gold standard dataset, and it is hard to evaluate the performance of our method. To overcome it, we first use Java source code as a dataset for our experiments, since it contains the namespace information. We verify that our method can partially recover namespaces from source code using only information about identifiers. The algorithms are evaluated on the English Wikipedia, and the proposed method can extract namespaces on a variety of topics. After extraction, the namespaces are organized into a hierarchical structure by using existing classification schemes such as MSC, PACS and ACM. We also apply it to the Russian Wikipedia, and the results are consistent across the languages. To our knowledge, the problem of introducing namespaces to mathematics has not been studied before, and prior to our work there has been no dataset where identifiers are grouped into namespaces. Thus, our result is not only a good start, but also a good indicator that automatic namespace discovery is possible.

==> 02formulaextraction.tex <==
\section{Mathematical Definition Extraction} \label{sec:definitionextraction-top}

In Natural Language Processing, Word Sense Disambiguation is a problem of 
identifying in which sense a polysemous word is used \cite{jurafsky2000speech}.
Analogously, the Identifier Disambiguation problem is a problem of 
determining the meaning of an identifier in a mathematical formula. This 
problem is typically solved by extracting definitions from the natural 
language description that surrounds the formula. 

For example, given the sentence ``The relation between energy and mass is
described by  the mass-energy equivalence formula $E = mc^2$,
where $E$ is energy, $m$ is mass and $c$ is the speed of light''
the goal is to extract the following identifier-definition relations:
($E$, ``energy''), ($m$, ``mass'') and
($c$, ``the speed of light'').


Formally, a phrase that defines a mathematical expression consists of three parts \cite{kristianto2012extracting}:

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
  \item \emph{definiendum} is the term to be defined: it is a mathematical expression
      or an identifier;
  \item \emph{definiens} is the definition itself: it is the word or phrase that defines the definiendum in a definition;
  \item \emph{definitor} is a relator verb that links definiendum and definiens.
\end{itemize}

In this work we are interested in the first two parts: \emph{definiendum} and
\emph{definiens}. Thus we define a \emph{relation} as a pair
(definiendum, definiens). For example, ($E$, ``energy'') is a relation where
$E$ is a definiendum, and ``energy'' is a definiens. We refer to definiendum as 
identifier, and to definiens as definition, so relations are identifier-definition
pairs. 

In this chapter we will discuss how the relations can be discovered automatically.
It is organized as follows: first, we discuss Part-of-Speech Tagging and its application
to mathematical texts in section~\ref{sec:postagging} and then 
review the extraction methods in section~\ref{sec:definition-extraction-methods}.


\subsection{Math-aware POS tagging} \label{sec:postagging}
Part-of-Speech Tagging (POS Tagging) is a typical Natural Language Processing
task which assigns a POS Tag to each word in a given text \cite{jurafsky2000speech}.
While the POS Tagging task is mainly a tool for text processing, it can
also be applicable to scientific documents with mathematical expressions,
and can be adjusted to dealing with formulae \cite{schoneberg2014pos}
\cite{pagael2014mlp}.

A \emph{POS tag} is an abbreviation that corresponds to some
part of speech. Penn Treebank POS Scheme \cite{santorini1990part} is
a commonly used POS tagging scheme which defines a set of part-of-speech tags
for annotating English words.
For example, \texttt{JJ} is an adjective (``big''), \texttt{RB} as in adverb,
\texttt{DT} is a determiner (``a'', ``the''), \texttt{NN} is a
noun (``corpus'') and \texttt{SYM} is used for symbols (``$>$'', ``$=$'').


However the Penn Treebank scheme does not have special tags for mathematics,
but it is flexible enough and can be extended to include additional tags.
For example, we can include a math-related tag \texttt{MATH}.
Usually it is done by first applying traditional POS taggers (like Stanford
CoreNLP \cite{manning2014stanford}), and then
refining the results by re-tagging math-related tokens of text as \texttt{MATH}
\cite{schoneberg2014pos}.


For example, consider the following sentence:
``The relation between energy and mass is
described by  the mass-energy equivalence formula $E = mc^2$,
where $E$ is energy, $m$ is mass and $c$ is the speed of light''.
In this case we will assign the \verb|MATH| tag to ``$E = mc^2$'', ``$E$'',
``$m$'' and ``$c$''

However we can note that for finding identifier-definition relations
the \texttt{MATH} tag alone is not sufficient: we need to distinguish
between complex mathematical expressions and stand-alone identifiers -
mathematical expressions that contain only one symbol: the identifier.
For the example above we would like to be able to distinguish the
expression ``$E = mc^2$'' from identifier tokens ``$E$'',
``$m$'' and ``$c$''. Thus we extend the Penn Treebank scheme even more
and introduce an additional tag \texttt{ID} to denote stand-alone identifiers.


Thus, in the example above ``$E = mc^2$'' will be assigned the \texttt{MATH} tag
and ``$E$'', ``$m$'' and ``$c$'' will be annotated with \texttt{ID}.

In the next section we discuss how this can be used to find identifier-definition
relations.


\subsection{Extraction Methods} \label{sec:definition-extraction-methods}
There are several ways of extracting the identifier-definition relations.
Here we will review the following:

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
  \item Nearest Noun
  \item Pattern Matching
  \item Machine-Learning based methods
  \item Probabilistic methods
\end{itemize}


\subsubsection{Nearest Noun Method}

\ \\

The Nearest Noun  \cite{grigore2009towards} \cite{yokoi2011contextual}
is the simplest definition extraction method.
It assumes that the definition is a combination of ad
It finds definitions by looking for combinations of adjectives and nouns
(sometimes preceded by determiners) in the text before the identifier.

I.e. if we see a token annotated with \texttt{ID}, and then a sequence
consisting only of adjectives (\texttt{JJ}), nouns (\texttt{NN}, \texttt{NNS})
and determiners (\texttt{DET}), then we say that this sequence is
the definition for the identifer.

For example, given the sentence ``In other words, the bijection $\sigma$ normalizes
$G$ in ...'' we will extract a relation ($\sigma$, "bijection").



\subsubsection{Pattern Matching Methods} \label{sec:pattern-matching}

\ \\

The Pattern Matching method \cite{quoc2010mining} is an extension of the
Nearest Noun method: In Nearest Noun, we are looking for one specific patten
where identifier is followed by the definition, but we can define several such
patterns and use them to extract definitions.

For example, we can define the following patterns:

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
  \item \texttt{IDE} \texttt{DEF}
  \item \texttt{DEF} \texttt{IDE}
  \item let$|$set \texttt{IDE} denote$|$denotes$|$be \texttt{DEF}
  \item \texttt{DEF} is$|$are denoted$|$\texttt{def}ined$|$given as$|$by \texttt{IDE}
  \item \texttt{IDE} denotes$|$denote$|$stand$|$stands as$|$by \texttt{DEF}
  \item \texttt{IDE} is$|$are \texttt{DEF}
  \item \texttt{DEF} is$|$are \texttt{IDE}
  \item and many others
\end{itemize}


In this method \texttt{IDE} and \texttt{DEF} are placeholders that are
assigned a value when the pattern is matched against some subsequence
of tokens.  \texttt{IDE} and DEF need to
satisfy certain criteria in order to be successfully matched: like in the
Nearest Noun method we assume that \texttt{IDE} is some token annotated with
\texttt{ID} and \texttt{DEF} is a phrase containing adjective (\texttt{JJ}),
nouns (\texttt{NN}) and  determiners (\texttt{DET}). Note that the first patten corresponds
to the Nearest Noun pattern.

The patterns above are combined from two lists: one is extracted from a 
guide to writing mathematical papers in English (\cite{trzeciak1995writing}), 
and another is extracted from ``Graphs and Combinatorics'' papers from Springer
\cite{kristianto2012extracting}. 

The pattern matching method is often used as the baseline method
for identifier-definition extraction methods \cite{kristianto2012extracting}
\cite{kristianto2014extracting} \cite{pagael2014mlp}.


\subsubsection{Machine Learning Based Methods}

\ \\

The definition extraction problem can be formulated as a binary classification
problem: given a pair (identifier, candidate-definition), does this pair
correspond to a real identifier-definition relation?

To do this we find all candidate pairs: identifiers are tokens
annotated with \texttt{ID}, and candidate defections are nouns and
noun phrases from the same sentence as the definition.

Once the candidate pairs are found, we extract the following features 
\cite{yokoi2011contextual} \cite{kristianto2014extracting}:


\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
  \item boolean features for each of the patterns from
    section~\ref{sec:pattern-matching} indicating if the pattern is matched,
  \item indicator if there's a colon or comma between candidate and identifier,
  \item indicator if there's another math expression between candidate and identifier,
  \item indicator if candidate is inside parentheses and identifier is outside,
  \item distance (in words) between the identifier and the candidate,
  \item the position of candidate relative to identifier,
  \item text and POS tag of one/two/three preceding and following tokens around the candidate,
  \item text of the first verb between candidate and identifier,
  \item many others.
\end{itemize}

Once the features are extracted, a binary classifier can be trained to predict
if an unseen candidate pair is a relation or not.
For this task the popular choices of classifiers are Support Vector Machine
classifier with linear kernel \cite{kristianto2014extracting} \cite{yokoi2011contextual}
and Conditional Random Fields \cite{kristianto2014extracting},
but, in principle, any other binary classifier can be applied
as well.


\subsubsection{Probabilistic Approaches} \label{sec:mlp} \ \\

In the Mathematical Language Processing approach \cite{pagael2014mlp}
a definition for an identifier is extracted by ranking
candidate definitions by the probability of definining
the identifier, and only the most probable candidates are retained.

The main idea of this approach is that the definitions occur very closely
to identifiers in sentences, and the closeness can be used to
model the probability distribution over candidate definitions.

The candidates are ranked by the following formula:
$$R(n, \Delta, t, d) = \cfrac{\alpha \, R_{\sigma_d}(\Delta) + \beta \, R_{\sigma_s}(n) + \gamma \, \text{tf}(t)}{\alpha + \beta + \gamma}$$
where $\Delta$ is the number of tokens between the identifier and the definition
candidate, and $R_{\sigma_d}(\Delta)$ is a Gaussian that models this distance, parametrized
with $\sigma_d$; $n$ is the number of sentences between the definition candidate 
and the sentence where the identifier occurs for the first time, and is a Gaussian
parameterized with $\sigma_s$; finally $\text{tf}(t)$ is a frequency of term $t$ 
in a sentence. All these quantities are combined together and $\alpha, \beta, \gamma$ are weighting parameters. 

The following weighting parameters $\alpha, \beta, \gamma$ are proposed in 
\cite{pagael2014mlp}: $\alpha = \beta = 1$ and $\gamma = 0.1$.



==> 06implementation.tex <==
\section{Implementation} \label{sec:implementation}


In section~\ref{sec:dataset} we describe the data set that we use,
then we describe how we extract identifiers from this dataset
(section~\ref{sec:defextraction-impl}) and how this dataset is cleaned
(section~\ref{sec:datacleaning}). Next, the implementation of clustering
algorithms is described in the section~\ref{sec:datacleaning}. After
the clusters are found, we combine them into a hierarchy in
the section~\ref{sec:hierarchy}.

Finally, in the section~\ref{sec:jlp} we explore how the same set of techniques
can be applied to source code in Java.


\subsection{Data set} \label{sec:dataset}

Wikipedia is a big online encyclopedia where the content
are written and edited by the community. It contains a large
amount of articles on a variety of topics, including articles about
Mathematics and Mathematics-related fields such as Physics. It
is multilingual and available in several languages, including
English, German, French, Russian and others. The content of wikipedia pages
are authored in a special markup language and the content of the entire
encyclopedia is freely available for download.


% why wiki?

The techniques discussed in this work are mainly applied
to the English version of Wikipedia. At the moment of writing
(\today) English Wikipedia contains about 4.9 million
articles\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Statistics}}.
However, just a small portion of these articles are math related:
there are only 30.000 pages that contain at least one \verb|<math>| tag.

Apart from the text data and formulas Wikipedia articles have information
about categories, and we can exploit this information as well.
The category information is encoded directly into each Wikipedia page
with a special markup tag. For example, the article
``Linear Regression''\footnote{\url{https://en.wikipedia.org/wiki/Linear_regression}}
belongs to the category ``Regression analysis'' and \verb|[[Category:Regression analysis]]|
tag encodes this information.
However there are other indirect ways to associate a page with some
category, for example, by using Wiki templates. A template is a user-defined macro
that is executed by the Wikipedia engine, and the content of a template
can include category association tags. It is hard
to extract the content information from the template tag and therefore
we use category information available in a structured
machine-processable form in DBPedia \cite{bizer2009dbpedia}.
Additionally, DBPedia provides extra information  such as parent
categories (categories of categories) that is very easy to process
and incorporate into analysis.


Wikipedia is available in other languages, not only English.
While the most of the analysis is performed on the English Wikipedia,
we also apply some of the techniques to the Russian version \cite{ruwikidump}
to compare it with the results obtained on English Wikipedia.
Russian Wikipedia is smaller that English Wikipedia and contains
1.9 million
articles\footnote{\url{https://en.wikipedia.org/wiki/Russian_Wikipedia}},
among which only 15\,000 pages are math-related (i.e. contain at
least one \verb|<math>| tag).


\subsection{Definition Extraction} \label{sec:defextraction-impl}

Before we can proceed to discovering identifier namespaces, we
need to extract identifier-definition relations. For this we use the probabilistic
approach, discussed in the section~\ref{sec:mlp}.
The extraction process is implemented using Apache Flink \cite{flink}
and it is based on the open source implementation provided by Pagael and
Schubotz in \cite{pagael2014mlp}\footnote{\url{https://github.com/rbzn/project-mlp}}.


The first step is to keep only mathematical articles and discard the rest.
This is done by retaining only those articles that contain
at least one \verb|<math>| tag. Once the data set is filtered, then
all the \LaTeX\ formulas form the \verb|<math>| tags are converted
to MathML, an XML-based representation of mathematical
formulae \cite{mathml}.

The dataset is stored in a big XML file in the Wiki XML
format. It makes it easy to extract the title and the content
of each document, and then process the documents separately.
The formulas are extracted by looking for the \verb|<math>| tags.
However some formulas for some reasons are typed without the tags
using the unicode symbols, and such formulas are very hard to
detect and therefore we choose not to process them.
Once all \verb|<math>| tags are found, they (along with the content)
are replaced with a special placeholder \verb|FORMULA_%HASH%|, where
\verb|%HASH%| is MD5 hash \cite{rivest1992md5} of the tag's content represented as
a hexadecimal string. After that
the content of the tags is kept separately from the document content.

The next step is to find the definitions for identifiers in formulas.
We are not interested in the semantics of a formula, only in the identifiers
it contains. In MathML \verb|<ci>| corresponds to identifiers, and
hence extracting identifiers from MathML formulas amounts to finding
all \verb|<ci>| tags and retrieving their content. It is enough to
extract simple identifiers such as ``$t$'', ``$C$'', ``$\mu$'', but
there also are complex identifiers with subscripts, such as
``$x_1$'', ``$\xi_i$'' or even ``$\beta_{\text{slope}}$''.
To extract them we need to look for tags \verb|<msub>|. We do not
process superscripts because they are usually powers (for example, ``$x^2$''),
and therefore they are not interesting for this work.
There are exceptions to this, for example, ``$\sigma^2$'' is an identifier,
but these cases are rare and can be ignored.

Since MathML is XML, the identifiers are extracted with XPath
queries \cite{moller2006introduction}:

\begin{itemize}
  \item \verb|//m:mi[not(ancestor::m:msub)]/text()| for all \verb|<ci>| tags
that are not subscript identifers;
  \item \verb|//m:msub| for subscript identifiers.
\end{itemize}

Once the identifiers are extracted, the rest of the formula is discarded.
As the result, we have a ``Bag of Formulae'': analogously to the Bag of Words
approach (see section~\ref{sec:vsm}) we keep only the counts of occurrences
of different identifiers and we do not preserve any other structure.


The content of Wikipedia document is authored with Wiki markup --
a special markup language for specifying document layout elements
such as headers, lists, text formatting and tables.
Thus the next step is to process the Wiki markup and extract the textual
content of an article, and this is done using a Java library
``Mylyn Wikitext'' \cite{mylynwikitext}.
Almost all annotations are discarded at this stage,
and only inner-wiki links are kept: they can be useful as candidate definitions.
The implementation of this step is taken entirely from \cite{pagael2014mlp}
with only a few minor changes.


Once the markup annotations are removed and the text content of an article is
extracted, we then apply Natural Language Processing (NLP) techniques.
Thus, the next step is the NLP step, and for NLP we use the
Stanford Core NLP library (StanfordNLP) \cite{manning2014stanford}.
The first part of this stage is to tokenize the text and also split it by sentences.
Once it is done, we then apply Math-aware POS tagging
(see section~\ref{sec:postagging}). For English documents from the English Wikipedia
we use StanfordNLP's Maximal Entropy POS Tagger \cite{toutanova2003feature}.
Unfortunately, there are no trained models available for POS tagging the Russian
language for the StanfordNLP library and we were not able to find a
suitable implementation of any other POS taggers in Java. Therefore we
implemented a simple rule-based POS tagger ourselves. The implementation is based on
a PHP function from \cite{habr2012postag}: it is translated into Java
and seamlessly integrated into the StanfordNLP pipeline.
The English tagger uses the Penn Treebank POS Scheme \cite{santorini1990part},
and hence we follow the same convention for the Russian tagger.


For handling mathematics we introduce two new POS classes:
``\verb|ID|'' for identifiers and ``\verb|MATH|'' for formulas.
These classes are not a part of the Penn Treebank POS Scheme,
and therefore we need to label all the instances of these tags ourselves
during the additional post-processing step. If a token starts
with ``\verb|FORMULA_|'', then we recognize that it is a placeholder
for a math formula, and therefore we annotate it with the ``\verb|MATH|''
tag. Additionally, if this formula contains only one identifier, this
placeholder token is replaced by the identifier and it is tagged with
``\verb|ID|''. We also keep track of all identifiers found in
the document and then for each token we check if this token is in the list.
If it is, then it is re-annotated with the ``\verb|ID|'' tag.

At the Wikipedia markup processing step we discard almost all markup
annotations, but we do keep inner Wikipedia links, because these links
are good definition candidates. To use them, we introduce
another POS Tag: ``\verb|LINK|''. To detect all inner-wiki links,
we first find all token subsequences that start with \verb|[[|
and end with \verb|]]|, and then these subsequences are
concatenated and tagged as ``\verb|LINK|''.

Successive nouns (both singular and plurals), possible modified
by an adjective, are also candidates for definitions. Therefore
we find all such sequences on the text and then concatenate each
into one single token tagged with ``\verb|NOUN_PHRASE|''.

The next stage is selecting the most probable identifier-definition
pairs, and this is done by ranking definition candidates.
The definition candidates are tokens annotated with ``\verb|NN|'' (noun singular),
``\verb|NNS|'' (noun plural), ``\verb|LINK|'' and ``\verb|NOUN_PHRASE|''.
We rank these tokens by a score that depends how far it is from the identifer
of interest and how far is the closest formula that contains this
identifier (see section~\ref{sec:mlp}).
The output of this step is a list of identifier-definition pairs along
with the score, and only the pairs with scores above
the user specified threshold are retained. The implementation of
this step is also taken entirely from \cite{pagael2014mlp} with very minor
modifications.

\subsubsection{Data Cleaning} \label{sec:datacleaning} \ \\

The Natural Language data is famous for being noisy and hard to
clean \cite{sonntag2004assessing}. The same is true for
mathematical identifiers and  scientific texts with formulas.
In this section we describe how the data was preprocessed and
cleaned at different stages of Definition Extraction.

Often identifiers contain additional semantic information visually conveyed
by special diacritical marks or font features. For example, the diacritics can be
hats to denote ``estimates'' (e.g. ``$\hat w$''), bars to denote the expected value
(e.g. ``$\bar X$''), arrows to denote vectors (e.g. ``$\vec x\, $'') and others.
As for the font features, boldness is often used to
denote vectors (e.g. ``$\mathbf w$'') or matrices (e.g. ``$\mathbf X$''), calligraphic fonts are
used for sets (e.g. ``$\mathcal H$''), double-struck fonts often denote spaces
(e.g. ``$\mathbb R$''), and so on.

Unfortunately there is no common notation established across all fields of
mathematics and there is a lot of variance. For example,
a vector can be denoted by ``$\vec x\, $'', ``$\boldsymbol x$'' or ``$\mathbf x$'',
and a real line by ``$\mathbb R$'', ``$\mathbf R$'' or ``$\mathfrak R$''.
In natural languages there are related problems of lexical ambiguity such as
synonymy, when different words refer to the same concept, and it can be solved
by replacing the ambiguous words with some token, representative of the concept.
Therefore this problem with identifiers can be solved similarly
by reducing identifiers to their ``root'' form. This can be done
by discarding all additional visual information, such that
``$\bar X$'' becomes ``$X$'', ``$\mathbf w$'' becomes ``$w$'' and ``$\mathfrak R$''
becomes ``$R$''. The disadvantage of this approach is that we lose
the additional semantic information about the identifier that overwise
could be useful.


The diacritic marks can easily be discarded because they are represented
by special MathML instructions that can be ignored when
the identifiers are retrieved. But, on the other hand,
the visual features are encoded directly on the character level:
the identifiers use special unicode symbols to convey font features such
as boldness or Fraktur, so it needs to be normalized by converting characters
from special ``Mathematical Alphanumeric Symbols'' unicode block \cite{allen2007unicode}
back to the standard ASCII positions (``Basic Latin'' block).
Some identifiers (such as ``$\hbar$'' or ``$\ell$'') are expressed using
characters from a special ``Letterlike Symbols'' table, and these characters
are normalized as well.

Additionally, the is a lot of noise on the annotation level in MathML formulas:
many non-identifiers are captures as identifiers inside \verb|<ci>| tags. Among
them there are many mathematic-related symbols
like ``\textasciicircum'', ``\#'',``$\forall$'', ``$\int$'';
miscellaneous symbols like ``$\diamond$'' or
``$\circ$'', arrows like ``$\to$'' and ``$\Rightarrow$'', and special characters like
``$\lceil$''.

To filter out these one-symbol false identifiers we fully exclude all characters from
the following unicode blocks: ``Spacing Modifier Letters'', ``Miscellaneous Symbols'',
``Geometric Shapes'', ``Arrows'', ``Miscellaneous Technical'', ``Box Drawing'',
``Mathematical Operators'' (except ``$\nabla$'' which is sometimes used as an identifier)
and ``Supplemental Mathematical Operators'' \cite{allen2007unicode}.
Some symbols (like ``='', ``+'', ``\verb|~|'', ``\%'', ``?'', ``!'')
belong to commonly used unicode blocks which we cannot exclude altogether.
For these symbols we manually prepare a stop list for filtering them.

It also captures multiple-symbol false positives: operator and function names
like ``\texttt{sin}'', ``\texttt{cos}'', ``\texttt{exp}'', ``\texttt{max}'', ``\texttt{trace}'';
words commonly used in formulas like ``\texttt{const}'', ``\texttt{true}'', ``\texttt{false}'',
``\texttt{vs}'', ``\texttt{iff}''; auxiliary words like ``\texttt{where}'',
``\texttt{else}'', ``\texttt{on}'', ``\texttt{of}'', ``\texttt{as}'', ``\texttt{is}'';
units like ``\texttt{mol}'', ``\texttt{dB}'', ``\texttt{mm}''.
These false identifiers are excluded by a stop list as well: if a
candidate identifier is in the list, it is filtered out.
The stop list of false positives is quite similar for
both English and Russian: for Russian wikipedia we only need
to handle the auxiliary words such as ``\texttt{где}'' (``\texttt{where}''),
``\texttt{иначе}'' (``\texttt{else}'') and so on. The names for operators and functions
are more or less consistent across both data sources.


Then, at the next stage, the definitions are extracted. However many
shortlisted definitions are either not valid definitions or too general.
For example, some identifiers become associated with ``\texttt{if and only if}'',
``\texttt{alpha}'', ``\texttt{beta}'', ``\texttt{gamma}'', which are not valid definitions.

Other definitions like ``\texttt{element}'' (``\texttt{элемент}''),
``\texttt{number}'' (``\texttt{число}'') or \\ ``\texttt{variable}'' (``\texttt{переменная}'' )
are valid, but they are too general and not descriptive. We maintain a stop list of such
false definitions and filter them out from the result. The elements
of the stop list are also consistent across both data data sets,
in the sense that the false definition candidates are same but expressed
in different languages.

The Russian language is highly inflected, and because of this extracted
definitions have many different forms, depending on grammatical gender,
form (singular or plural) and declensions. This highly increases the
variability of the definitions, and to reduce it lemmatize the definitions:
they are reduced to the same common form (nominative, singular and masculinum).
This is done using Pymorphy2: a python library for Russian and
Ukrainian morphology \cite{korobov2015morphological}.

At the next stage the retrieved identifier/definition pairs
are used for document clustering. Some definitions are used only
once and we can note that they are not very useful because
they do not have any discriminative power. Therefore all such
definitions are excluded.


\subsubsection{Dataset Statistics}  \ \\

At the identifier extraction step when the data set is cleaned,
some identifiers are discarded, and after that some documents
become empty: they no longer contain any identifiers, and which is why
these documents are not considered for further analysis.
Additionally, we discard all the documents that have only one identifier.
This leaves only 22\,515 documents out of 30\,000, and they
contain 12\,771 distinct identifiers, which occur about 2 million times.

The most frequent identifiers are ``$x$'' (125\,500 times), ``$p$'' (110\,000),
``$m$'' (105\,000 times) and ``$n$'' (83\,000 times), but about 3\,700 identifiers occur
only once and 1\,950 just twice. Clearly, the distribution of
identifiers follows some power law distribution (see fig.~\ref{fig:ed-wiki-ids}).

\begin{figure}[h]
\centering
\hfill
\begin{subfigure}[b]{0.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{en-wiki-ids-1.pdf}
  \caption{Frequencies of the first 50 identifiers}
  \label{fig:en-wiki-ids-1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{en-wiki-ids-2-log.pdf}
  \caption{Frequencies, log scale}
  \label{fig:en-wiki-ids-2-log.pdf}
\end{subfigure}
\hfill
\caption{Distribution of frequencies of identifiers}
\label{fig:ed-wiki-ids}
\end{figure}



The distribution of counts for identifiers inside the documents also
appears to follow a long tail power law distribution: there are few articles
that contain many identifiers, while most of the articles do not
(see fig.~\ref{fig:en-wiki-doc-ids-1.pdf}).
The biggest article (``Euclidean algorithm'') has 22\,766 identifiers, a
and the second largest (``Lambda lifting'') has only 6\,500 identifiers.
The mean number of identifiers per document is 33.
The distribution for number of distinct identifiers per document
is less skewed (see fig.~\ref{fig:en-wiki-doc-ids-2.pdf}).
The largest number of distinct identifiers is 287 (in the article
``Hooke's law''), and it is followed by 194 (in ``Dimensionless quantity'').
The median number of identifiers per document is 10.


\begin{figure}[h]
\centering

\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{en-wiki-doc-ids-1.pdf}
  \caption{Identifier frequencies per document for first 80 most largest documents}
  \label{fig:en-wiki-doc-ids-1.pdf}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{en-wiki-doc-ids-2.pdf}
  \caption{No. of distinct identifiers per document for first 80 most largest documents}
  \label{fig:en-wiki-doc-ids-2.pdf}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{en-wiki-doc-def.pdf}
  \caption{Definitions per document}
  \label{fig:en-wiki-doc-def.pdf}
\end{subfigure}

\caption{Frequencies per documents}
\label{fig:freqs-doc}

\end{figure}


For 12\,771 identifiers the algorithm extracted 115\,300 definitions, and the
number of found definitions follows a long tail distribution as well
(see fig.~\ref{fig:en-wiki-doc-def.pdf}), with the median number of
definitions per page being 4.

The following is the list of the most common identifier-definition pairs
extracted from English Wikipedia:

\begin{itemize}
\item $t$: ``time'' (1086)
\item $m$: ``mass'' (424)
\item $\theta$: ``angle'' (421)
\item $T$: ``temperature'' (400)
\item $r$: ``radius'' (395)
\item $v$: ``velocity'' (292)
\item $\rho$: ``density'' (290)
\item $G$: ``group'' (287)
\item $V$: ``volume'' (284)
\item $\lambda$: ``wavelength'' (263)
\item $R$: ``radius'' (257)
\item $n$: ``degree'' (233)
\item $r$: ``distance'' (220)
\item $c$: ``speed of light'' (219)
\item $L$: ``length'' (216)
\item $n$: ``length'' (189)
\item $n$: ``order'' (188)
\item $n$: ``dimension'' (185)
\item $n$: ``size'' (178)
\item $M$: ``mass'' (171)
\item $d$: ``distance'' (163)
\item $X$: ``topological space'' (159)
\end{itemize}

In Russian Wikipedia only 5\,300 articles contain enough identifiers,
and the remaining 9\,500 are discarded.

The identifiers and definitions extracted from the Russain version of
Wikipedia exhibit the similar properties. The most frequently
occurring identifier is ``$x$'' with 13\,248 occurrences,
but the median frequency of an identifer is only 3 times.
The article with the largest number of identifiers is ``Уравнения Максвелла''
(``Maxwell's equations'') which contains 1\,831 identifiers, while
the median number of identifiers is just 3;
the article with the largest number of distinct identifiers
is also  ``Уравнения Максвелла'' with 112 unique identifiers, and
the median number of distinct identifiers in the data set is 5.
Finally, the largest number of extracted definitions is 44
(again, for ``Уравнения Максвелла'') with 2 being the median number of
definitions per page.

The following is the list most frequent relations extracted
from Russian wikipedia:

\begin{itemize}
\item $t$: ``функция'' (``function'') (215)
\item $t$: ``время'' (``time'') (130)
\item $X$: ``множество'' (``set'') (113)
\item $m$: ``масса'' (``mass'') (103)
\item $c$: ``скорость свет'' (``speed of light'') (89)
\item $G$: ``группа'' (``group'') (87)
\item $T$: ``температура'' (``temperature'') (69)
\item $h$: ``постоянный планка'' (``Plank constant'') (68)
\item $\rho$: ``плотность'' (``density'') (57)
\item $M$: ``многообразие'' (``manifold'') (53)
\item $K$: ``поль'' (``field'') (53)
\item $X$: ``пространство'' (``space'') (50)
\item $v$: ``скорость'' (``speed'') (50)
\item $X$: ``топологический пространство'' (``topological space'') (46)
\item $G$: ``граф'' (``graph'') (44)
\item $R$: ``радиус'' (``radius'') (38)
\item $R$: ``кольцо'' (``ring'') (36)
\item $G$: ``гравитационный постоянный'' (``gravitational constant'') (34)
\item $E$: ``энергия'' (``energy'') (34)
\item $m$: ``модуль'' (``modulo'') (33)
\item $S$: ``площадь'' (``area'') (32)
\item $k$: ``постоянный больцмана'' (``Boltzmann constant'') (30)
\end{itemize}



\subsection{Document Clustering} \label{sec:clustering-impl}

At the Document Clustering stage we want to find cluster of documents
that are good namespace candidates.

Before we can do this, we need to vectorize our dataset: i.e. build the
Identifier Space (see section~\ref{sec:vsm}) and represent each document
in this space.

There are three choices for dimensions of the Identifier space:

\begin{itemize}
  \item identifiers alone,
  \item ``weak'' identifier-definition association,
  \item ``strong'' association: use identifier-definition pairs.
\end{itemize}

In the first case we are only interested in identifier information and
discard the definitions altogether.

In the second and third cases we keep the definitions and use them to
index the dimensions of the Identifier Space. Bur there is some
variability in the definitions: for example, the same identifier
``$\sigma$'' in one document can be assigned to ``Cauchy stress tensor'' and
in other it can be assigned to ``stress tensor'', which are almost the same thing.
To reduce this variability we perform some preprocessing: we tokenize
the definitions and use individual tokens to index dimensions of the space.
For example, suppose we have two pairs ($\sigma$, ``Cauchy stress tensor'')
and ($\sigma$, ``stress tensor''). In the ``weak'' association case
we have will dimensions $(\sigma, \text{Cauchy}, \text{stress}, \text{tensor})$,
while for the ``strong'' association case we will have
$(\sigma\text{\_Cauchy}, \sigma\text{\_stress}, \sigma\text{\_tensor})$.

Additionally, the effect of variability can be decreased further
by applying a stemming technique for each definition token.
In this work we use Snowball stemmer for English \cite{porter2001snowball}
implemented in NLTK \cite{bird2006nltk}: a python library for
Natural Language Processing. For Russian we use Pymorphy2 \cite{korobov2015morphological}.

Using \verb|TfidfVectorizer|  from  scikit-learn \cite{scikit-learn} we vectorize
each document. The experiments are performed with $\log \text{TF} \times \text{IDF}$ weighting,
and therefore we use \verb|use_idf=False, sublinear_tf=True| parameters
for the vectorizer. Additionally, we use \verb|min_df=2| to discard identifiers
that occurs only once.

The output is a document-identifier matrix (analogous to ``document-term''):
documents are rows and identifiers/definitions are columns.
The output of \verb|TfidfVectorizer| is row-normalized, i.e. all rows has unit length.

Once we the documents are vectorized, we can apply clustering techniques
to them. We use $K$-Means (see section~\ref{sec:kmeans}) implemented as a
class \verb|KMeans| in scikit-learn and Mini-Batch $K$-Means (class \verb|MiniBatchKMeans|) \cite{scikit-learn}. Note that if rows are unit-normalized, then running $K$-Means with
Euclidean distance is equivalent to cosine distance
(see section~\ref{sec:cosine}).

% TODO: uncomment if use it during the experiments
%Bisecting $K$-Means (see section~\ref{sec:kmeans}) was implemented on top of
%scikit-learn: at each step we take a subset of the dataset and apply
%$K$-Means with $K = 2$ to this subset. If the subset is big (with number of
%documents $n > 2000$), then we use Mini-Batch $K$-means with $K=2$
%because it converges much faster.


DBSCAN (section~\ref{sec:dbscan}) and SNN Clustering (also section~\ref{sec:dbscan})
algorithms were %also
implemented manually: available DBSCAN implementations usually take distance
measure rather than a similarity measure. The similarity matrix cleated by similarity measures
are typically very sparse, because usually only a small fraction of the documents
are similar to some given document. Similarity measures
can be converted to distance measures, but in this case
the matrix will no longer be sparse, and we would like to avoid that.
Additionally, available implementations are usually general purpose
implementations and do not take advantage of the structure of the data:
in text-like data clustering algorithms can be sped up significantly
by using an inverted index.


Dimensionality reduction techniques are also important: they
not only reduce the dimensionality, but also help reveal the latent
structure of data. In this work we use Latent Semantic Analysis (LSA) (section~\ref{sec:lsa})
which is implemented using randomized Singular Value Decomposition (SVD)
\cite{tropp2009finding}, The implementation of randomized SVD is taken from scikit-learn
\cite{scikit-learn} -- method \verb|randomized_svd|. Non-negative Matrix Factorization
is an alternative technique for dimensionality reduction (section~\ref{sec:lsa}).
Its implementation is also taken from scikit-learn \cite{scikit-learn},
class \verb|NMF|.

To assess the quality of produced clusters we use wikipedia categories. It is
quite difficult to extract category information from raw wikipedia text,
therefore we use DBPedia \cite{bizer2009dbpedia} for that: it provides
machine-readable information about categories for each wikipedia article.
Additionally, categories in wikipedia form a hierarchy, and this hierarchy
is available as a SKOS ontology.

Unfortunately, there is no information about articles from Russian Wikipedia on
DBPedia. However the number of documents is not very large, and therefore
this information can be retrieved via MediaWiki API\footnote{\url{http://ru.wikipedia.org/w/api.php}} individually for each
document. This information can be retrieved in chunks for a group of several
documents at once, and therefore it is quite fast.

\subsubsection{Building Namespaces} \ \\

Once a cluster analysis algorithm assigns documents in our collection to
some clusters, we need to find namespaces among these clusters. We assume that
some clusters are namespace-defining: they are not only homogenous in the cluster
analysis sense (for example, in case of $K$-Means it means that within-cluster sum
of squares is minimal), but also ``pure'': they are about the same topic.

A cluster is \emph{pure} if all documents belong to the same category.
Using categories information we can find the most frequent category of the
cluster, and then we can define purity of a cluster $C$ as
$$\operatorname{purity}(C) = \cfrac{\max_i \operatorname{count}(c_i)}{|C|},$$
where $c_i$'s are cluster categories.
Thus we can select all clusters with purity above some pre-defined threshold
and refer to them as namespace-defining clusters.

Then we convert these clusters into namespaces by collecting all the identifiers
and their definitions in the documents of each cluster. To do this, we first
collect all the identifier-definition pairs, and then group them by identifier.
When extracting, each definition candidate is scored, and this score is used
to determine, which definition an identifier will be assigned in the namespace.

For example, consider three documents with the following extracted relations:

\begin{itemize}
  \item Document A:
  \begin{itemize}
\item $n$: (predictions, 0.95), (size, 0.92), (random sample, 0.82), (population, 0.82)
\item $\theta$: (estimator, 0.98), (unknown parameter, 0.98), (unknown parameter, 0.94)
\item $\mu$: (true mean, 0.96), (population, 0.89)
\item $\mu_4$: (central moment, 0.83)
\item $\sigma$: (population variance, 0.86), (square error, 0.83), (estimators, 0.82)
  \end{itemize}

  \item Document B:
    \begin{itemize}
\item $P_\theta$: (family, 0.87)
\item $X$: (measurable space, 0.95)
\item $\theta$: (sufficient statistic, 0.93)
\item $\mu$: (mean, 0.99), (variance, 0.95), (random variables, 0.89), (normal, 0.83)
\item $\sigma$: (variance, 0.99), (mean, 0.83)
  \end{itemize}

  \item Document C:
    \begin{itemize}
\item $n$: (tickets, 0.96), (maximum-likelihood estimator, 0.89)
\item $x$: (data, 0.99), (observations, 0.93)
\item $\theta$: (statistic, 0.95), (estimator, 0.93), (estimator, 0.93), (rise, 0.91), (statistical model, 0.85), (fixed constant, 0.82)
\item $\mu$: (expectation, 0.96), (variance, 0.93), (population, 0.89)
\item $\sigma$: (variance, 0.94), (population variance, 0.91), (estimator, 0.87)
  \end{itemize}
\end{itemize}

We take all these relations, and combine together. If an identifer
have two or more definitions that are exactly the same, them we
merge them into one and its score is the sum of scores:

\begin{itemize}
\item $P_\theta$: (family, 0.87)
\item $X$: (measurable space, 0.95), (Poisson, 0.82)
\item $n$: (tickets, 0.96), (predictions, 0.95), (size, 0.92), (maximum-likelihood estimator, 0.89), (random sample, 0.82), (population, 0.82)
\item $x$: (data, 0.99), (observations, 0.93)
\item $\theta$: (estimator, 0.98+0.93+0.93), (unknown parameter, 0.98+0.94), (statistic, 0.95), (sufficient statistic, 0.93), (rise, 0.91), (statistical model, 0.85), (fixed constant, 0.82)
\item $\mu$: (random variables, 0.89+0.89+0.89), (variance, 0.95+0.93), (mean, 0.99), (true mean, 0.96), (expectation, 0.96), (normal, 0.83)
\item $\mu_4$: (central moment, 0.83)
\item $\sigma$: (variance, 0.99+0.94), (population variance, 0.91+0.86), (estimator, 0.87), (square error, 0.83), (mean, 0.83), (estimators, 0.82)
\end{itemize}

There is some lexical variance in the definitions. For example, ``variance'' and ``population
variance'' or ``mean'' and ``true mean'' are very related definitions, and
it makes sense to group them together to form one definition.
It can be done by fuzzy string matching (or approximate matching)
\cite{navarro2001guided}. To implement it, we use a python library FuzzyWuzzy
\cite{fuzzywuzzy}, and using fuzzy matching we group related identifiers and then
sum over their scores.

Then we have the following:

\begin{itemize}
\item $P_\theta$: (family, 0.87)
\item $X$: (measurable space, 0.95), (Poisson, 0.82)
\item $n$: (tickets, 0.96), (predictions, 0.95), (size, 0.92), (maximum-likelihood estimator, 0.89), (random sample, 0.82), (population, 0.82)
\item $x$: (data, 0.99), (observations, 0.93)
\item $\theta$: (estimator, 2.84), (unknown parameter, 1.92), (\{statistic, sufficient statistic\}, 1.88), (rise, 0.91), (statistical model, 0.85), (fixed constant, 0.82)
\item $\mu$: (random variables, 2.67), (\{mean, true mean\}, 1.95), (variance, 1.88),  (expectation, 0.96), (normal, 0.83)
\item $\mu_4$: (central moment, 0.83)
\item $\sigma$: (\{variance, population variance\}, 3.7), (\{estimator, estimators\}, 1.69), (square error, 0.83), (mean, 0.83)
\end{itemize}

In a namespace an identifier can have at most one definition, and therefore the next step
is selecting the definition with the highest score. This gives us the following namespace:

\begin{itemize}
\item ($P_\theta$, family, 0.87)
\item ($X$, measurable space, 0.95)
\item ($n$, tickets, 0.96)
\item ($x$, data, 0.99
\item ($\theta$, estimator, 2.84)
\item ($\mu$, random variables, 2.67)
\item ($\mu_4$, central moment, 0.83)
\item ($\sigma$: variance, 3.7)
\end{itemize}


The category of this namespace is selected as the category that the majority of the documents
in the namespace-defining cluster share.


\subsection{Experiments} \label{sec:param-tuning}

There are many different clustering algorithms, each with its own set
of parameter. In this section we describe how we find the settings that
find the best namespaces.

The following things can be changed:

\begin{itemize}
  \item Ways to incorporate definition information (no definitions, soft association, hard association);
  \item Weighting schemes for the identifier-document matrix $D$: TF, sublinear TF, TF-IDF;
  \item There are different clustering algorithms: agglomerative clustering, DBSCAN, SNN
  clustering, $K$-Means, %Bisecting $K$-Means,
  and each algorithm has its own set of parameters;
  \item Dimensionality of $D$ can be reduced via SVD or NMF, parameter $k$ controls the
      rank of output.
\end{itemize}

% The approach for finding
% Distance and similarity measures used
% Euclidean distance, cosine similarity, jaccard similarity, SNN Similarity

To find the best parameters set we use the grid search approach: we try
different combinations of parameters and keep track on the number of
pure clusters and the purity.

The overall purity of cluster assignment is calculated as a weighed sum
of individual  cluster purities, where the weight is chosen proportionally to
the size of a cluster.

\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.75\textwidth}
  \centering\includegraphics[width=\textwidth]{purity.pdf}
  \caption{Number of clusters $K$ vs overall purity of clustering:
      the purity increases linearly with $K$ ($R^2 = 0.99$).}
  \label{fig:k-vs-purity}
\end{subfigure}
\begin{subfigure}[b]{0.75\textwidth}
  \centering\includegraphics[width=\textwidth]{pure-clusters.pdf}
  \caption{Number of clusters $K$ vs the number of pure clusters: it grows initially, but after $K\approx 8\,000$ starts to decrease.}
  \label{fig:k-vs-pureclusters}
\end{subfigure}
\caption{Purity and number of pure clusters as measures of algorithm performance.}
\label{fig:performace}
\end{figure}

However it is not enough just to find the most pure cluster assignment: because
as the number of clusters increases the overall purity also grows.
Thus we can also optimize for the number of clusters with purity $p$ of
size at least $n$.
When the number of clusters increase, the purity always grows
(see fig.~\ref{fig:k-vs-purity}), but at some point the number of pure clusters
will start decreasing (see fig.~\ref{fig:k-vs-pureclusters}).



\subsubsection{Baseline} \ \\

We compare the performance of clustering algorithms against a random
categorizer. The simplest version of such a categorizer is the random
cluster assignment categorizer, which assigns each document to some random
cluster.
In this case, we constrain the categorizer to include 3 documents in each
cluster, and once a document belongs to some cluster, it cannot be re-assigned.
It is done by first creating a vector of assignments and shuffling it.

Then we record how many pure clusters (at least 80\% pure) are in the cluster
assignment.

\begin{figure}[h!]
\centering\includegraphics[width=0.7\textwidth]{baseline.pdf}
\caption{Distribution of the number of pure clusters across 200 trials.}
\label{fig:baseline}
\end{figure}

To establish the baseline, we repeated this experiment for 200
times (see fig.~\ref{fig:baseline}), and the maximal achieved value is 39 pure
clusters, while the mean value is 23.85.


% \textbf{TODO }Also: experiment with not just three, but with some
% probability distribution say clusters can vary from 3 to 10 or whatever.



\subsubsection{Only Identifiers} \ \\

The first way of building the identifier space is to use only identifiers
and do not use definitions at all.

If we do this, the identifier-document matrix is $6075 \times 22512$
(we keep only identifiers that occur at least twice), and it contains  302\, 541
records, so the density of this matrix is just 0.002.

First, we try to apply agglomerative clustering, then DBSCAN with SNN similarity
based on Jaccard coefficient and cosine similarity, then we
do $K$-Means and finally we apply LSA using SVD and NMF and apply
$K$-Means on the reduced space.


\begin{figure}[h!]
\centering\includegraphics[width=0.75\textwidth]{agglo-time.pdf}
\caption{Runtime of agglomerative clustering is quadratic with the number of documents
in the collection ($R^2 = 0.99$).}
\label{fig:agglo-time}
\end{figure}

\textbf{Agglomerative clustering} algorithms are quite fast for small datasets,
but they become more computationally expensive as the dataset size grows.
We run a series of experiments on subsamples of our dataset and we can observe that the run
time is quadratic with the number of documents to cluster
(see fig.~\ref{fig:agglo-time}). The polynomial regression model that we built predicts
that it should process the entire dataset of 22\,512 documents in 90 minutes,
but it was not able to finish in several hours, so we stopped the computation.
Additionally, the implementation we use from scikit-learn
requires a dense matrix. But when densified, the identifier-document matrix
occupies a lot of space: if each element of the matrix is represented with a double 
precision number, then this matrix occupies 1.01 Gb of RAM in total. While 
it is small enough to fit into memory, matrices of larger dimensionality might not.
Therefore we exclude these clustering algorithms from further analysis.
% Agglomerative: Wald linkage: takes forever never finished


\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-jac10.pdf}
  \caption{Number of clusters when 10 nearest neighbors are considered}
  \label{fig:nodef-dbscan-jac10}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-jac10-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 10 nearest neighbors}
  \label{fig:nodef-dbscan-jac10-2}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-jac13.pdf}
  \caption{Number of clusters when 15 nearest neighbors are considered}
  \label{fig:nodef-dbscan-jac15}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-jac13-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 15 nearest neighbors}
  \label{fig:nodef-dbscan-jac15-2}
\end{subfigure}
\caption{Effect of parameters $\varepsilon$, \texttt{MinPts} and number of nearest
 neighbors on performance of SNN DBSCAN when Jaccard coefficient is used.}
\label{fig:nodef-dbscan-jac}
\end{figure}

The second method is \textbf{DBSCAN} with \textbf{SNN Similarity}.
To compute SSN similarity we need to use some other base similarity measure.
We start with Jaccard coefficient, and use a binarized identifier-document
matrix: a matrix with only ones and zeros.
For example, the closest article to ``Linear Regression'' is
``Linear predictor function'' with Jaccard coefficient of 0.59
and ``Low-rank approximation'' is the closest to ``Singular value decomposition''
with coefficient of 0.25. With Jaccard, we were able to discover 87
clusters, which is two times better than the baseline (see fig.~\ref{fig:nodef-dbscan-jac})
and the best parameters are 10 nearest neighbors,
$\varepsilon=3$ and \texttt{MinPts} $=4$ (see fig.~\ref{fig:nodef-dbscan-jac10-2}).


For the best result with 87 namespace defining clusters,
in total 5\,580 clusters were found and 4\,219 documents are considered
as ``noise''. Let us consider top largest found clusters (see table~\ref{tab:nodef-jaccard}).
One of them, ``Statistics'',  is quite homogenous with purity of 0.84 (see table~\ref{tab:nodef-jaccard-stat}).
Although some of the articles in this cluster are not related to statistics,
all of them articles share the same identifier ``$\beta$''.
We can also check how $\beta$ is defined across all namespace-defining clusters
(see table~\ref{tab:nodef-jaccard-beta}). There are not many instance of
$\beta$, and not all of them correct or meaningful: for example  ``i/ab'' in
the ``Physics'' cluster is a non-definition that was not successfully filtered
out during the data cleaning phase.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Name & Size & Purity \\
  \hline
Continuum mechanics & 40 & 0.8000 \\
Constellations listed by Ptolemy & 17 & 1.0000 \\
Statistics & 13 & 0.8462 \\
Knot theory & 13 & 0.8462 \\
Electromagnetism & 12 & 0.8333 \\
Bayer objects & 11 & 1.0000 \\
Analytic number theory & 10 & 0.9000 \\
Acoustics & 9 & 0.8889 \\
Chemical properties & 9 & 0.8889 \\
Set theory & 9 & 0.8889 \\
Combinatorics & 8 & 0.8750 \\
Theory of computation & 8 & 1.0000 \\
Partial differential equations & 8 & 0.8750 \\
Mathematical logic & 8 & 0.8750 \\
\hline
\end{tabular}
\caption{Top namespace-defining clusters discovered by SNN DBSCAN with Jaccard coefficient.}
\label{tab:nodef-jaccard}
\end{table}

\begin{table}[h!]
\centering
\begin{subtable}{0.65\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
Article Name & Identifiers \\
\hline
Partition of sums of squares & $y, \beta_0, \beta_1, \varepsilon_i, \beta_p, S, \varepsilon, y_i, \beta, ...$ \\
Deming regression & $\sigma, \eta, \eta_i, \beta, \beta_0, \varepsilon_i, \varepsilon, \delta, y_i, x, ...$ \\
Instrumental variable & $\beta, \varepsilon, \delta, x_1, Y, X,g, f, \varepsilon_i, \beta_k, ...$ \\
Ordinary least squares & $w_i, \alpha, \beta, \varepsilon, \sigma, E, \eta, \chi, \varepsilon_i,  \beta_j, ...$ \\
Endogeneity & $\gamma, \varepsilon_i, \beta_1, x_i, \alpha, \beta, \varepsilon, ...$ \\
Linear predictor function & $x_i, \varepsilon_2, \beta_0,  \varepsilon_1, \beta, \varepsilon, \phi_p, \varepsilon_n, ...$ \\
Stochastic frontier analysis & $\beta_n, f, \beta_0, u_i, x_i, \beta, T, y_i, ...$ \\
\begin{tabular}[x]{@{}c@{}} Proofs involving \\ ordinary least squares \end{tabular} &
  $x_i, \beta_0, \beta_1, \beta, \varepsilon, \pi, \sigma, \chi, \varepsilon_i, ...$ \\
Projection pursuit regression & $\beta, \beta_0, j, S, \varepsilon, y_i, X, Y, x, x_i, ...$ \\
De Casteljau's algorithm & $w_i, \beta_0, \beta_1,  \beta, \beta_i, t, \beta_n, t_0, P_0, ...$ \\
Regression analysis & $x_i, \beta_0, \beta, \varepsilon, y_i, \sigma, f, \beta_p, \varepsilon_i, ...$ \\
Linear regression & $x_i, \varepsilon_2, \Omega, \beta_1, \beta_2, y_n, \varepsilon_1, \beta, \varepsilon, ...$ \\
Least squares & $\nabla, \beta_j, \beta, \varepsilon, w_{ii}, Wy, \sigma, \varepsilon_i, ...$ \\
\hline
\end{tabular}
\label{tab:nodef-jaccard-docs}
\caption{Identifiers and articles of the ``Statistics'' cluster (some identifiers are removed)}
\end{subtable}% mask EOL
\begin{subtable}{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ID & Definition & Score\\
\hline
$X_1$ & regressors & 0.92 \\
$Y$ & regression model & 0.95 \\
$f$ & linear predictor function & 0.99 \\
$p$ & regressors & 1.77 \\
$w_i$ & control points & 1.66 \\
$y_0$ & mean response & 0.99 \\
$y_i$ & dependent variable & 3.71 \\
$z$ & causal relationship & 0.90 \\
$\alpha$ & confidence level & 1.94 \\
$\beta$ & estimator & 2.82 \\
$\beta_1$ & slope & 1.82 \\
$\varepsilon$ & errors & 2.90 \\
$\varepsilon_i$ & error term & 2.71 \\
$\sigma$ & residual variance & 2.68 \\
\hline
\end{tabular}
\label{tab:nodef-jaccard-ids}
\caption{Definitions in ``Statistics'' (some definitions are removed)}
\end{subtable}
\caption{A namespace-defining cluster about Statistics dicovered by SNN DBSCAN
with Jaccard coefficient.}
\label{tab:nodef-jaccard-stat}
\end{table}



\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  \multicolumn{4}{|c|}{$\beta$}\\
  \hline
  Size & Namespace Name & Definition & Score \\
  \hline
3 & Complex analysis & absolute value & 0.95 \\
40 & Continuum mechanics & bias & 1.75 \\
5 & Fluid dynamics & momentum factor & 0.95 \\
5 & Physics & i/ab & 0.84 \\
3 & Quantum mechanics & voltage-to-barrier-field conversion factor & 1.87 \\
5 & Radio frequency propagation & clutter factor & 0.95 \\
9 & Set theory & successor ordinal & 0.89 \\
13 & Statistics & estimator & 2.82 \\
6 & Theoretical physics & quantity & 0.96 \\
\hline
\end{tabular}
\caption{Definitions of ``$\beta$'' in the namespaces discovered by SNN DBSCAN with Jaccard coefficient.}
\label{tab:nodef-jaccard-beta}
\end{table}




Then we run the same algorithm, but with cosine similarity, using an
identifier-document matrix with $(\log \text{TF}) \times \text{IDF}$
weights, and calculate pair-wise similarity between each document.
For example, let us take an article ``Linear regression''
%it contains $h_i, m, n, p, T, t, t_i, X, x, x_{11},$ $x_{21}, x_i, y, y_1,$
%$y_2, y_i, y_n, Z,  \beta, \beta_1, \beta_2, \beta_p, \varepsilon, \varepsilon_1,
%\varepsilon_2,$ $\varepsilon_i, \varepsilon_n, \Omega$
and calculate the cosine with the rest of the corpus. The closest document
is ``Linear predictor function''.
% with identifiers
%$b, c, c_1, f, m, p1, T, x, X,$ $x_{11}, x_i, x_K, y, y_2, y_i, y_n, \beta_0,
%\beta_1, \beta_2, \beta_p, \beta 2, \varepsilon,$ $\varepsilon_1, \varepsilon_2, \varepsilon_i,$
%$\phi, \phi_1, \phi_2$.
They have 23 identifiers in common, and they indeed look related.
However cosine is not always giving the best closets neighbors. For example,
the nearest neighbor of ``Singular value decomposition'' is ``Rule of Sarrus'',
and although their cosine score is 0.92, they have only 3 identifiers in common.

\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-cos10.pdf}
  \caption{Number of clusters when 10 nearest neighbors are considered}
  \label{fig:nodef-dbscan-cos10}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-cos10-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 10 nearest neighbors}
  \label{fig:nodef-dbscan-cos10-2}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-cos15.pdf}
  \caption{Number of clusters when 15 nearest neighbors are considered}
  \label{fig:nodef-dbscan-cos15}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{nodef-dbscan-cos15-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 15 nearest neighbors}
  \label{fig:nodef-dbscan-cos15-2}
\end{subfigure}
\caption{Effect of parameters $\varepsilon$, \texttt{MinPts} and number of nearest
 neighbors on performance of SNN DBSCAN when cosine is used.}
\label{fig:nodef-dbscan-cos}
\end{figure}


With cosine as the base similarity function for SNN DBSCAN we
were able to discover 124 namespace-defining clusters (see fig.~\ref{fig:nodef-dbscan-cos}),
which is significantly better than the baseline. The best parameters
are 10 nearest neighbors and $\varepsilon=4$, \texttt{MinPts} $=3$
(see fig.~\ref{fig:nodef-dbscan-cos10-2}).


\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.75\textwidth}
  \centering\includegraphics[width=\textwidth]{k-vs-time.pdf}
  \caption{$K$ in $K$-Means vs time in minutes ($R^2 = 0.99$).}
  \label{fig:k-vs-time}
\end{subfigure}

\begin{subfigure}[b]{0.75\textwidth}
  \centering\includegraphics[width=\textwidth]{k-vs-time-minibatch.pdf}
  \caption{$K$ in MiniBatch $K$-Means vs time in seconds ($R^2 = 0.97$).}
  \label{fig:k-vs-time-minibatch}
\end{subfigure}
\caption{Runtime of $K$-Means and MiniBatch $K$-Means}
\label{fig:kmeans-vs-minibatch1}
\end{figure}

Next, we apply \textbf{$K$-Means}. We observe that increasing~$K$
leads to linear increase in time (see fig.~\ref{fig:k-vs-time}),
which means that for bigger values of~$K$, it takes longer, so it is not
feasible to run: for example, we estimate the runtime of $K$-Means with $K = 10\, 000$
to be about 4.5 hours. As \textbf{MiniBatch $K$-Means} is expected to be significantly
faster than usual $K$-Means, we use it as well. Although we observe that the run
time of  MiniBatch $K$-Means also increases linearly with~$K$
(see fig.~\ref{fig:k-vs-time-minibatch}), it indeed runs considerably faster.
For example, MiniBatch $K$-Means takes 15 seconds with $K=700$ while
usual $K$-Means takes about 15 minutes (see fig.~\ref{fig:k-vs-time}
and fig.~\ref{fig:k-vs-time-minibatch}).


\begin{figure}[h!]
\centering
\hfill
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{k-vs-purity2.pdf}
  \caption{Purity vs number of clusters $K$ in \mbox{$K$-Means} and MiniBatch $K$-Means}
  \label{fig:k-vs-purity2}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{k-vs-len2.pdf}
  \caption{Number of pure clusters vs $K$ in $K$-Means and MiniBatch $K$-Means}
  \label{fig:k-vs-len2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{\textwidth}
  \centering
  \includegraphics[width=0.85\textwidth]{k-vs-len-mb.pdf}
  \caption{Number of pure clusters vs $K$ in MiniBatch $K$-Means for larger $K$}
  \label{fig:k-vs-len-mb}
\end{subfigure}
\hfill
\caption{Effect of $K$ on performance in $K$-Means}
\label{fig:kmeans-vs-minibatch}
\end{figure}


Usual $K$-Means with small $K$ does not find many good and pure clusters,
and MiniBatch $K$-Means does even worse: no matter what $K$ is selected,
the number of pure clusters and purity does not change much (see fig.~\ref{fig:k-vs-purity2}
and fig.~\ref{fig:k-vs-len2}). This is also true for larger values of $K$
(see fig.~\ref{fig:k-vs-len-mb}).


% to the end of subsubsection?
%We can conclude that although MiniBatch $K$-Means is
%very fast, it does not perform well on the untransformed data when we don't use
%definitions.


The best result was found by usual $K$-Means with $K=600$: it was able
to discover 19 clusters with purity at least 0.8 (note that this is worse
than the baseline of 39 pure clusters). Although it is not many,
the found clusters are very tight and quite big.
Among others, it discovered the following clusters: ``Astronomical catalogues'' (53 documents)
``Stochastic processes'' (39 documents), ``Theory of computation'' (17 documents),
``Thermodynamics'' (16 documents), ``Statistics'' (13 documents).
For example, the cluster ``Astronomical catalogues'' (see table~\ref{tab:kmeans-stars})
primarily constants documents about stars, and all these documents share
the same set of identifers $(p, R_*, m, R_\odot)$.

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
Article & Identifiers \\
\hline
Beta Columbae & $p, R_*, m, R_\odot$ \\
Eta Pegasi & $p, R_*, m, R_\odot$ \\
Sigma Puppis & $p, R_*, m, R_\odot$ \\
Gamma Ceti & $p, R_*, m, R_\odot$ \\
Epsilon Corvi & $p, R_*, m, R_\odot$ \\
Beta Corvi & $p, R_*, m, R_\odot$ \\
Gamma Herculis & $p, R_*, m, R_\odot$ \\
Psi2 Aurigae & $p, R_*, m, R_\odot$ \\
Psi7 Aurigae & $p, R_*, m, R_\odot$ \\
Epsilon Sagittarii & $p, R_*, m, R_\odot$ \\
Alpha Gruis & $p, R_*, m, R_\odot$ \\
Theta Centauri & $p, R_*, m, R_\odot$ \\
... & ... \\
\hline
\end{tabular}
\caption{Stars cluster discovered by $K$-Means.}
\label{tab:kmeans-stars}
\end{table}

Next, we use \textbf{Latent Semantic Analysis} with \textbf{SVD}
to reduce the dimensionality of the identifier-document
matrix $D$, and then apply $K$-Means on the reduced space. As discussed in the
LSA section (see section~\ref{sec:lsa}), it should reveal the latent structure of data.
Hence, we expect that it should improve the results achieved by usual $K$-Means.

\begin{figure}[h!]
\centering\includegraphics[width=0.75\textwidth]{k-svd-vs-time.pdf}
\caption{Effect of $k$ in $k$-rank-reduced randomized SVD on the runtime in seconds.}
\label{fig:k-svd-vs-time}
\end{figure}


Randomized SVD is very fast, but the runtime does not grow linearly with $k$,
it looks quadratic (see fig.~\ref{fig:k-svd-vs-time}).
However, the typical values of $k$ for SVD used in latent semantic analysis is
150-250 \cite{aggarwal2012survey} \cite{evangelopoulos2012latent},
therefore the run time is not prohibitive, and we do not need to rut it
with very large $k$.

\begin{figure}[h!]
\centering
\hfill
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{k-vs-mb-svd-purity.pdf}
  \caption{Purity vs number of clusters $K$ in \mbox{$K$-Means} and MiniBatch $K$-Means.}
  \label{fig:k-vs-mb-svd-purity}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{k-vs-mb-svd-len.pdf}
  \caption{Number of pure clusters vs $K$ in $K$-Means and MiniBatch $K$-Means.}
  \label{fig:k-vs-mb-svd-len}
\end{subfigure}
\caption{The performance of $K$-Means and MiniBatch $K$-Means on the reduced document space with $k=150$.}
\label{fig:kmeans-vs-minibatch-svd}
\end{figure}


When the dimensionality is reduced, the performance of $K$-Means and
MiniBatch $K$-Means is similar (see fig.~\ref{fig:k-vs-mb-svd-purity}),
but with MiniBatch $K$-Means we were able to discover more interesting pure
clusters (see fig.~\ref{fig:k-vs-mb-svd-len}). The reason for this may be the fact that in the reduced space there is less noise and both methods find equally good clusters,
but because MiniBatch $K$-Means works faster, we are able to run it multiple
times thus increasing its chances to find a good local optimum where there
are many pure document clusters. Note that the obtained result is below
the baseline.

We can observe that as $K$ increases, the number of interesting clusters increases
(see fig.~\ref{fig:k-vs-mb-svd-len}).
Therefore, we try a wide range of larger $K$ for different $k \in \{150, 250, 350, 500\}$.
The performance in terms of discovered pure clusters does not depend much on the
rank $k$ of the reduced space (see fig.~\ref{fig:k-vs-kmeans-len-nodef}). In fact,
it is very hard to distinguish different lines because they are quite perplexed.
The maximum for is achieved at $K \approx 10000$ for all $k$.

\begin{figure}[h!]
\centering\includegraphics[width=0.9\textwidth]{k-vs-kmeans-len-nodef.pdf}
\caption{Number of discovered pure clusters in $K$-Means for different number of clusters $K$ and rank $k$.}
\label{fig:k-vs-kmeans-len-nodef}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Name & Size & Purity \\
  \hline
Astronomical catalogues & 53 & 0.9811 \\
Quantum mechanics & 14 & 0.9286 \\
Electrochemistry & 12 & 0.8333 \\
Particle physics  & 10 & 0.8000 \\
Partial differential equations  & 10 & 0.8000 \\
Electromagnetism  & 10 & 1.0000 \\
Topology  & 10 & 0.9000 \\
Measure theory  & 8 & 0.8750 \\
Propositional calculus  & 8 & 0.8750 \\
Baseball statistics  & 7 & 0.8571 \\
Group theory  & 7 & 0.8571 \\
Abstract algebra & 6 & 0.8333 \\
\hline
\end{tabular}
\caption{Top namespace-defining clusters discovered by $K$-Means with $K=9500$ on LSA-space with $k=250$}
\label{tab:nodef-kmeans-lsa}
\end{table}

A clustering obtained with $K=9500$ and $k=250$ discovered 213 namespace-defining
clusters (see table~\ref{tab:nodef-kmeans-lsa}), which is significantly better
than the baseline. Let us consider a namespace
defined by the Measure Theory cluster with 8 documents, where 7 articles in
this cluster are from ``Measure theory'' category, and all the documents share
the ``$\mu$'' identifier (see table~\ref{tab:nodef-kmeans-lsa-measuretheory}).

\begin{table}[h!]
\centering
\begin{subtable}{0.65\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
Article Name & Identifiers \\
\hline
Signed measure & $\Sigma, E, d, f, l, n, P, R, t, x, N, \nu, \mu$ \\
Ergodicity & $\Sigma,E,g,H,n,T,X,\mu, t$ \\
Support (measure theory) & $\Sigma,D,g,f,C,T,L,R,U,t,\lambda,\mu,d$ \\
Convergence of measures & $d,g,f,\mu_n,l,n,P,S,R,\eta,t,\nu,\mu$ \\
\begin{tabular}[x]{@{}c@{}} Riesz–Markov–Kakutani \\ representation theorem \end{tabular}
   & $E,d,f,\psi,K,\alpha,U,X,x,\mu$ \\
Invariant measure & $\Sigma, B,\phi,f,\mu,S,R,t,x,b,T$ \\
Fernique's theorem & $E,l_*,G,k,l,\alpha,t,x,\mu,d$ \\
Gauge symmetry & $E,d_\nu,J,L,U,W,\nu,\mu$ \\
\hline
\end{tabular}
\label{tab:nodef-kmeans-lsa-measuretheory-docs}
\caption{Identifiers and articles of the ``Measure Theory'' cluster (some identifiers are removed)}
\end{subtable}% mask EOL
\begin{subtable}{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ID & Definition & Score\\
\hline
$C$ & closed set & 0.95 \\
$f$ & measurable function & 3.50 \\
$t$ & measurable & 1.64 \\
$\Sigma$ & sigma algebra & 1.86 \\
$\alpha$ & form & 0.87 \\
$\lambda$ & measure & 0.96 \\
$\mu$ & measure & 11.16 \\
$\mu_n$ & measure & 0.97 \\
$\nu$ & nonnegative measure & 0.96 \\
$\phi$ & monoid & 0.91 \\
$\psi$ & positive linear functional & 1.89 \\
\hline
\end{tabular}
\label{tab:nodef-kmeans-lsa-measuretheory-ids}
\caption{Definitions in ``Measure Theory'' (some definitions are removed)}
\end{subtable}
\caption{A namespace-defining cluster about Measure Theory discovered by $K$-Means
with $K=9500$ and $k=250$}
\label{tab:nodef-kmeans-lsa-measuretheory}
\end{table}


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  \multicolumn{4}{|c|}{$\mu$}\\
  \hline
  Size & Namespace Name & Definition & Score \\
  \hline
7 & Baseball statistics & dissociation constant & 0.89 \\
5 & Bletchley Park & motor wheels & 4.51 \\
3 & Continuous distributions & mean & 4.52 \\
5 & Fluid dynamics & dynamic viscosity & 0.99 \\
3 & Force & entropy & 0.93 \\
3 & Force & permeability & 3.63 \\
5 & General relativity & vierbein field & 0.95, \\
3 & General relativity & reduced mass & 1.79 \\
3 & Machine learning & hyperparameter & 0.86 \\
5 & Mathematical analysis & measure & 3.69 \\
5 & Mathematical finance & brownian motion & 0.84 \\
8 & Measure theory & measure & 11.16 \\
6 & Measure theory & assumptions & 0.93 \\
3 & Mechanics & modulus & 0.89 \\
3 & Molecular physics & absorption coefficient & 0.95 \\
5 & Orbits & semi-major axis & 0.89 \\
4 & Physics & numerator & 0.95 \\
4 & Probability distributions & ratio & 0.96 \\
4 & Probability theory & mean & 0.95 \\
6 & Quantum field theory & gamma matrices & 1.73 \\
14 & Quantum mechanics & molecular dipole operator & 0.96 \\
4 & Quantum mechanics & magnetic moment & 0.97 \\
3 & Quantum mechanics & magnetic dipole moment & 0.9 \\
5 & Quantum mechanics & chemical potential & 0.96 \\
3 & Quantum mechanics & formal limit & 0.95 \\
4 & Set theory & order type & 0.97 \\
3 & Special functions & partitions & 0.99 \\
3 & Stars & angular rate & 0.96 \\
6 & Statistical theory & true mean & 1.79 \\
3 & Statistical theory & standard deviation & 1.90 \\
4 & Stochastic processes & expectation & 0.96 \\
3 & Stochastic processes & time t & 0.99 \\
4 & Structural engineering & kinetic energy & 0.93 \\
6 & Theoretical physics & covariant derivative & 0.89 \\
4 & Theory of relativity & expression a\_$\mu$b & 0.93 \\
3 & Theory of relativity & four-velocity & 0.87 \\
3 & Thermodynamics & chemical potential & 1.88 \\
\hline
\end{tabular}
\caption{Definitions of $\mu$ in the namespaces discovered by $K$-Means with $K=9500$
and SVD with $k=250$ (some identifier/definition pairs are removed).}
\label{tab:nodef-kmeans-mu}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Name & Size & Purity \\
  \hline
Astronomical catalogues  & 53 & 0.9811 \\
Complex analysis  & 18 & 0.8333 \\
Quantum mechanics  & 12 & 0.8333 \\
Mathematical analysis  & 10 & 0.8000 \\
Physics  & 9 & 0.8889 \\
Thermodynamics  & 6 & 0.8333 \\
Astronomical catalogues of stars  & 6 & 1.0000 \\
Knot theory  & 6 & 1.0000 \\
Stochastic processes  & 6 & 1.0000 \\
Physics  & 6 & 0.8333 \\
Stochastic processes  & 6 & 1.0000 \\
Statistics  & 6 & 0.8333 \\
\hline
\end{tabular}
\caption{Top namespace-defining clusters discovered by $K$-Means with $K=9500$ on NMF-space with $k=250$.}
\label{tab:nodef-nmf}
\end{table}

It is also interesting to look at all the occurrences of ``$\mu$'' in
the results, and see how it is defined
across different namespace-defining cluster (see table~\ref{tab:nodef-kmeans-mu}).
We can note several problems. First, sometimes there are namespaces with the same
name, but ``$\mu$'' stands for different things there, for example, for namespaces
``Force'' probably either ``entropy'' or ``permeability'' is not assigned correctly.
Second, there are clearly incorrect definitions such as ``assumptions''
for the ``Measure theory'' namespace. Also, there are non-definitions such
as ``expression a\_$\mu$b'' or ``time t'' assigned to $\mu$. And finally,
some namespaces are questionable, e.g. ``Bletchley Park''. But overall
it does discover many definitions correctly, for example, ``measure'',
``mean'', ``expectation'' and others.

\begin{table}[h!]
\centering
\begin{subtable}{0.65\textwidth}
\centering
\begin{tabular}{|c|c|}
\hline
Article Name & Identifiers \\
\hline
Pivotal quantity & $\zeta,\theta,\nu,\mu,\rho,\sigma,N,X_2,X_1,x,z,...$ \\
Errors and residuals & $\sigma,\chi,X_n,\epsilon_i,X_i,n,X_1,X,N,\mu,S_n,...$ \\
Prediction interval & $\epsilon_i,X_i,\alpha,\gamma,\beta,\mu,s_n,\sigma,E,\Phi,...$ \\
Cochran's theorem & $\mu,\sigma,B,\chi,R,U,T,Y,X,k,j,Q_2,Q_1,...$ \\
Skewness & $\gamma,m_3,\kappa,\nu,\mu,\sigma,E,F,s,u,t,...$ \\
Variance & $\Sigma, \text{SS}_\text{within},\theta,\lambda,\mu,\rho,\sigma,E,f,...$ \\
\hline
\end{tabular}
\caption{Identifiers and articles of the ``Measure Theory'' cluster (some identifiers are removed).}
\label{tab:nodef-nmf}
\end{subtable}% mask EOL
\begin{subtable}{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ID & Definition & Score\\
\hline
$E$ & non-central moment & 0.92 \\
$F$ & cumulative distribution function & 0.89 \\
$f$ & probability density function & 0.99 \\
$s$ & sample variance & 3.66 \\
$\lambda$ & exponential distribution & 1.79 \\
$\mu$ & variance & 3.52 \\
$\rho$ & correlation & 0.99 \\
$\sigma$ & standard deviation & 4.61 \\
\hline
\end{tabular}
\caption{Definitions in ``Measure Theory'' (some definitions are removed).}
\label{tab:nodef-nmf-def}
\end{subtable}
\caption{A namespace-defining cluster about Measure Theory discovered by $K$-Means
with $K=9500$ and SVD with $k=250$.}
\label{tab:nodef-nmf-stat}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  \multicolumn{4}{|c|}{$\mu$}\\
  \hline
  Size & Namespace Name & Definition & Score \\
  \hline
4 & Abstract algebra & lebesgue measure & 0.83 \\
4 & Algebraic curves & first & 0.93 \\
3 & Condensed matter physics & magnetic permeability & 0.99 \\
3 & Coordinate systems & form & 1.81 \\
3 & Differential equations & invariant measure & 2.73 \\
3 & Doppler effects & spatial resolution & 0.95 \\
6 & Dynamical systems & tent map & 1.71 \\
5 & Dynamical systems & entropy & 0.93 \\
6 & Electromagnetism & permeability & 1.90 \\
4 & Electromagnetism & gauge condition & 0.99 \\
4 & Financial markets & drift rate & 0.89 \\
3 & Force & th-component & 0.95 \\
3 & Functions and mappings & lebesgue measure & 0.91 \\
3 & Gravitation & semi-major axis & 0.89 \\
3 & Group theory & tate module & 1.76 \\
3 & Magnetism & magnetic moment & 1.90 \\
5 & Measure theory & measure & 8.15 \\
6 & Multivariable calculus & measure & 1.82 \\
5 & Numerical analysis & step size & 0.93 \\
6 & Physical chemistry & chemical potential & 2.57 \\
3 & Probability distributions & confidence interval & 2.77 \\
3 & Probability distributions & laplace & 3.42 \\
3 & Probability distributions & scale factor & 1.84 \\
4 & Probability theory & mean & 0.95 \\
5 & Quantum field theory & field & 0.81 \\
12 & Quantum mechanics & gamma matrices & 1.78 \\
6 & Quantum mechanics & magnetic moment & 0.87 \\
3 & Quantum mechanics & mass & 0.89 \\
3 & Solid state engineering & charge & 0.93 \\
6 & Statistical theory & known mean & 0.99 \\
6 & Statistics & variance & 3.52 \\
3 & Statistics & mean & 1.85 \\
6 & Stochastic processes & time t & 0.99 \\
6 & Stochastic processes & free rate & 0.95 \\
3 & Stochastic processes & expectation & 0.96 \\
5 & Systems theory & earths gravity & 0.93 \\
3 & Telecommunications engineering & yield & 0.93 \\
4 & Theories of gravitation & indices & 1.94 \\
3 & Theory of relativity & velocity component & 0.93 \\
\hline
\end{tabular}
\caption{Definitions of $\mu$ in the namespaces discovered by $K$-Means with $K=9500$
and NMF with $k=250$ (some identifier/definition pairs are removed).}
\label{tab:nodef-nmf-mu}
\end{table}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{nmf-runtime.pdf}
\caption{Runtime of NMF for different $k$.}
\label{fig:nmf-runtime}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{k-vs-kmeans-len-nmf-nodef.pdf}
\caption{Number of discovered pure clusters in $K$-Means and NMF for different number of clusters $K$ and rank $k$.}
\label{fig:k-vs-kmeans-len-nmf-nodef}
\end{figure}

We also can apply \textbf{Non-Negative Matrix Factorization} for LSA.
NMF takes significantly more time than randomized SVD (see fig.~\ref{fig:nmf-runtime}).
In addition, although the runtime should be $O(nk)$ \cite{xu2003document}, we do not
observe that it grows linearly with $k$. On the contrary, it appears that there is rather
quadratic relationship. We expected that the results produced by NMF will
be better than SVD because of non-negativity of produced results,
but the performance is quite similar (see fig.~\ref{fig:k-vs-kmeans-len-nmf-nodef}).
For NMF, however, it is easier to see the difference in performance when different rank $k$ is used, and the curves are not as perplexed as for SVD. We see that $k=250$ does better on
$K=[8000; 12000]$ than $k=150$ and $k=350$. For example, $K$-Means with
$K=9500$ and $k=250$ discovered a clustering with 200 namespace-defining clusters.
The found clusters are slightly different. For example, there is no ``Measure Theory''
cluster of size 8 as in the results, found by SVD (see table~\ref{tab:nodef-kmeans-lsa}).
Let us instead consider a namespace defined by the cluster ``Statistics''
(see table~\ref{tab:nodef-nmf-stat}): there are 6 documents in the cluster
(see table~\ref{tab:nodef-nmf}) and about 43 identifier-definition in the namespace
defined by this cluster (see table~\ref{tab:nodef-nmf-def}).
Note that ``$\mu$'' is not assigned correctly in this cluster: it is defined as
``variance'' instead of ``mean''. If we look at all definitions of ``$\mu$''
in this clustering (see table~\ref{tab:nodef-nmf-mu}) we see that, although the problems
are the same as with decomposition by SVD, the found definitions are different.
However the difference is likely to be because of non-convexity of $K$-Means
rather than some crucial difference in the way the matrix are factorized.


We also see that generally clustering works better on reduced spaces.


\begin{figure}[h!]
\centering\includegraphics[width=0.9\textwidth]{nodef-weighing.pdf}
\caption{The effect of using different weighting systems on $K$-Means with SVD.}
\label{fig:nodef-weighing}
\end{figure}


In the experiments above we used the $(\log \text{TF}) \times \text{IDF}$ weighting scheme.
Let us compare the effect of different weighting on the resulting clusters.
To do that, we apply SVD  with $k=150$ and run MiniBatch $K$-Means for a set of smaller $K$'s
because it is computationally faster. We can observe that performance of $K$-Means
does not depend significantly on the weighting system when no definitions
are used (see fig.~\ref{fig:nodef-weighing}).



\subsubsection{Weak Association} \ \\

The identifier-document matrix has the dimensionality $10419 \times 22512$,
and there are 485\,337 elements in the matrix, so the density is about 0.002.


\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{soft-dbscan-cos10.pdf}
  \caption{Number of clusters when 10 nearest neighbors are considered}
  \label{fig:soft-dbscan-cos10}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{soft-dbscan-cos10-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 10 nearest neighbors}
  \label{fig:soft-dbscan-cos10-2}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{soft-dbscan-cos13.pdf}
  \caption{Number of clusters when 15 nearest neighbors are considered}
  \label{fig:soft-dbscan-cos15}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{soft-dbscan-cos13-2.pdf}
  \caption{Performance of selected $\varepsilon$ with 15 nearest neighbors}
  \label{fig:soft-dbscan-cos15-2}
\end{subfigure}
\caption{Effect of parameters $\varepsilon$, \texttt{MinPts} and number of nearest
 neighbors on performance of SNN DBSCAN when cosine is used.}
\label{fig:soft-dbscan-cos}
\end{figure}

We do not attempt to use hierarchical methods and start with DBSCAN. Previously we have
observed that Jaccard is inferior to cosine similarity, and therefore we start directly
with cosine.

Like in no-definition case, we calculate the cosine similarity on document vectors
where elements are weighed with $(\log \text{TF}) \times \text{IDF}$. Using definitions
it gives better results, than just identifiers. For example,
for ``Linear regression'' the closest document is ``Linear predictor function'' with
cosine of 0.62, which is the same result, obtained when no definitions are used.
However, for ``Singular value decomposition'' the most similar document is
``Moore–Penrose pseudoinverse'' with cosine score of 0.386, and this is more meaningful
than the most similar document when no definitions are used.
As previously, we applied \textbf{SNN DBSCAN} with 10 and 15 nearest neighbors, and the best
result was obtained with 10 nearest neighbors, $\varepsilon=3$ and \texttt{MinPts}$=3$
(see fig.~\ref{fig:soft-dbscan-cos}). It was able to discover 223 namespace-defining
clusters, which is slightly better than the best case when no definitions are
used.

With  \textbf{MiniBatch $K$-Means} applied on the plain untransformed document
space we are able to find some interesting clusters, but it general, similarity to the no-definition case, the does not show good results overall. Therefore we
apply it to the LSA space reduced by \textbf{SVD}, when identifier-document matrix
is reduced to rank $k$. We search for
the best combination trying $K = [500; 15000]$ and $k \in \{150, 250, 350\}$.
Unlike the case where no definitions are used, the space produced by the
soft definition association is affected by $k$ (see fig.~\ref{fig:k-vs-kmeans-len-svd-soft})
and the results produced by $k = 350$ are almost always better.
The weighing scheme used for this experiment is $(\log \text{TF}) \times \text{IDF}$.


\begin{figure}[h!]
\centering\includegraphics[width=0.9\textwidth]{k-vs-kmeans-len-svd-soft.pdf}
\caption{Number of discovered pure clusters in $K$-Means and SVD for different number of clusters $K$ and rank $k$.}
\label{fig:k-vs-kmeans-len-svd-soft}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Name & Size & Purity \\
  \hline
Astronomical catalogues & 53 & 0.9811 \\
Statistics & 20 & 0.8500 \\
Category theory & 16 & 0.8125 \\
Electromagnetism & 12 & 0.8333 \\
Thermodynamics & 11 & 0.8182 \\
Mathematical analysis & 11 & 0.8182 \\
Graph theory & 10 & 0.9000 \\
Graph algorithms & 10 & 0.8000 \\
Fluid dynamics & 10 & 1.0000 \\
Numerical analysis & 9 & 0.8889 \\
Group theory & 9 & 1.0000 \\
Stochastic processes & 9 & 1.0000 \\
Measure theory & 8 & 1.0000 \\
\hline
\end{tabular}
\caption{Top namespace-defining clusters discovered by $K$-Means with $K=9750$ on LSA-space with $k=350$}
\label{tab:soft-kmeans-svd}
\end{table}

\begin{table}[h!]
\centering
\begin{subtable}{0.7\textwidth}
\centering
\begin{tabular}{|c|c|}
  \hline
  Article & Identifiers \\
  \hline
Diagonalizable matrix & $v_1,\lambda_1,v_k,\lambda_3,\lambda_2,\lambda_i,\lambda_k,\lambda_j,\lambda_n,...$\\
Eigenvalues and eigenvectors & $v_i,\mu_A,\lambda_i,d,\lambda_n,...$ \\
Principal axis theorem & $v_1,u_1,\lambda_1,\lambda_2,D,S,u,...$ \\
Eigendecomposition of a matrix & $\lambda,\lambda_1,\lambda,\lambda_2,\lambda_k,R,U,T,...$ \\
Min-max theorem & $\sigma,u_n,u_k,u_i,u_1,\alpha,\lambda_1,\lambda,\lambda_i,...$ \\
Linear independence & $\Lambda,v_j,u_2,v_3,u_n,\lambda_1,\lambda_3,\lambda_2,...$ \\
Symmetric matrix & $\Lambda,\lambda_1,\lambda_2,D,Q,P,\lambda_i,...$ \\
\hline
\end{tabular}
\caption{Wiki Articles in the cluster ``Linear Algebra''}
\label{tab:soft-kmeans-la}
\end{subtable}% mask EOL
\begin{subtable}{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ID & Definition & Score\\
\hline
$D$ & diagonal matrix & 1.81 \\
$t$ & real argument & 0.99 \\
$u$ & eigenvalues & 0.89  \\
$u_i$ & eigenvector & 0.89  \\
$v_1$ & eigenvectors & 1.86  \\
$\Lambda$ & diagonal matrix & 2.65  \\
$\lambda$ & eigenvalue & 0.85 \\
$\lambda_1$ & eigenvalues & 3.66 \\
$\lambda_2$ & eigenvalues & 1.76 \\
$\lambda_3$ & eigenvalues & 0.83 \\
$\lambda_i$ & eigenvalue & 4.40 \\
\hline
\end{tabular}
\caption{Definitions in ``Linear Algebra''}
\label{tab:soft-kmeans-la-def}
\end{subtable}
\caption{A ``Linear Algebra'' cluster found by $K$-Means with $K=9000$ and $k=250$.}
\label{tab:soft-kmeans-lsa}
\end{table}

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  \multicolumn{4}{|c|}{$\lambda$}\\
  \hline
  Size & Namespace Name & Definition & Score \\
  \hline
3 & Algebra & multiplicity & 0.93 \\
4 & Analysis of variance & marquardt & 1.71 \\
3 & Applied and interdisciplinary physics & wavelength & 4.52 \\
6 & Cartographic projections & longitude & 10.02 \\
3 & Cartography & longitude & 7.24 \\
3 & Category theory & natural isomorphisms & 0.84 \\
4 & Condensed matter physics & penetration depth & 0.95 \\
5 & Continuous distributions & affine parameter & 0.99 \\
3 & Coordinate systems & longitude & 2.74 \\
3 & Differential equations & differential operator & 0.89 \\
8 & Differential geometry & vector fields & 1.82 \\
7 & Electronic amplifiers & typical value & 0.93 \\
3 & Electrostatics & unit length & 0.93 \\
10 & Fluid dynamics & wavelength & 6.44 \\
6 & Fluid dynamics & free path & 0.93 \\
3 & Infinity & limit ordinals & 2.68 \\
7 & Linear algebra & eigenvalue & 0.85 \\
5 & Linear algebra & matrix & 0.87 \\
3 & Linear algebra & eigenvalue & 2.53 \\
3 & Liquids & relaxation time & 0.88 \\
3 & Materials science & rate & 0.95 \\
3 & Mathematical analysis & eigenvalue & 0.86 \\
3 & Mathematical theorems & poisson distribution & 0.87 \\
4 & Measure theory & lebesgue measure & 0.95 \\
3 & Measurement & order & 0.89 \\
8 & Mechanics & previous expression & 0.95 \\
4 & Mechanics & power series & 0.88 \\
3 & Metalogic & empty word & 0.96 \\
7 & Number theory & partition & 1.90 \\
4 & Number theory & modular lambda function & 0.99 \\
3 & Operator theory & algebraic multiplicity & 0.95 \\
5 & Optics & wavelength & 1.76 \\
5 & Partial differential equations & constants & 0.87 \\
4 & Physical optics & wavelength & 3.59 \\
5 & Physics & exciton state & 2.76 \\
6 & Probability distributions & references & 0.89 \\
4 & Quantum field theory & coupling constant & 1.94 \\
5 & Quantum mechanics & wavelength & 6.47 \\
5 & Quantum mechanics & state & 2.66 \\
3 & Radioactivity & decay & 1.82 \\
4 & Representation theory of Lie groups & weight & 7.11 \\
3 & Riemannian geometry & contravariant vector field & 0.96 \\
4 & Rubber properties & engineering strain & 8.96 \\
3 & Statistical data types & regularization parameter & 0.96 \\
20 & Statistics & words & 0.93 \\
3 & Statistics & expectation & 0.99 \\
3 & Stellar astronomy & mean free path & 0.92 \\
3 & Surface chemistry & ideal gas & 0.83 \\
3 & Theoretical physics & eigenvalue & 2.71 \\
5 & Theories of gravitation & dicke & 0.95 \\
3 & Wave mechanics & wavelength & 2.65 \\
\hline
\end{tabular}
\caption{Some of definitions of ``$\lambda$'' in the clustering obtained with $K$-Means.}
\label{tab:soft-kmeans-lambda}
\end{table}

The best result in this scheme is 414 namespace-defining clusters
(ten times better than the baseline), and it is achieved by $K$-Means
with $K=9750$ and $k=350$. The purity of this clustering is $0.63$.
Let us consider a ``Linear Algebra'' cluster (table~\ref{tab:soft-kmeans-lsa})
with 6 documents and some of extracted definitions in documents
of this cluster, and all these articles share identifers $\lambda_1$, $m$ and $n$.
Let us consider all definitions of identifier ``$\lambda$''. In total, there
are 93 clusters where ``$\lambda$'' is used (see table~\ref{tab:soft-kmeans-lambda}),
and in many cases it is possible to determine that the assignment is correct
(e.g. ``eigenvalue'', ``wavelength'', ``regularization parameter'').
Some cases are not correct, for example, when we have clusters with the same name
where $\lambda$ denotes different things (e.g. in two ``Quantum Mechanics'' clusters),
or in the case of ``Linear Algebra'' cluster where it denotes a matrix.


\begin{figure}[h!]
\centering\includegraphics[width=0.9\textwidth]{k-vs-kmeans-len-nmf-soft.pdf}
\caption{The effect of rank $k$ used in NMF on $K$-Means.}
\label{fig:nnmf-soft}
\end{figure}

\textbf{Non-Negative Matrix Factorization} gives good results, but does not improve on
the best result obtained with SVD (see fig.~\ref{fig:nnmf-soft}).
The largest number of namespace-defining clusters is 370 and it is achieved
with $K=10000$ and $k=350$.


\begin{figure}[h!]
\centering\includegraphics[width=0.9\textwidth]{soft-weighing.pdf}
\caption{The effect of using different weighting systems on $K$-Means with SVD
($k=150$).}
\label{fig:soft-weighing}
\end{figure}


We also experiment with different weighting schemes, and, unlike the no-definition
case, it has a significant effect on the results: we can observe that sublinear
TF is better that untransformed TF, and $(\log \text{TF}) \times \text{IDF}$
achieves the best performance (see fig.~\ref{fig:soft-weighing}).




\subsubsection{Strong Association} \ \\

$37879 \times 22512$ sparse identifier-document matrix with 499070 entries,
so the density of this matrix is just 0.00058.

\textbf{DBSCAN?}

Like for the soft association case, we choose not to perform usual $K$-Means,
and instead proceed directly to MiniBatch $K$-Means on the LSA space
reduced with SVD. With rank $k=500$ and number of clusters $K = 8250$
is achieves the best result of 340 clusters (see fig.~\ref{fig:k-vs-kmeans-len-svd-strong}),
which is slightly worse than in the weak association case. The purity
of obtained clustering is 0.5683.

\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{k-vs-kmeans-len-svd-strong.pdf}
\caption{Number of discovered pure clusters in $K$-Means and SVD for different number of clusters $K$ and rank $k$.}
\label{fig:k-vs-kmeans-len-svd-strong}
\end{figure}

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Name & Size & Purity \\
  \hline
Astronomical catalogues & 53 & 0.9811 \\
Set theory & 10 & 0.9000 \\
Propositional calculus & 10 & 0.8000 \\
Group theory & 10 & 0.8000 \\
Electromagnetism & 9 & 0.8889 \\
Rotation & 9 & 0.8889 \\
Numerical analysis & 9 & 0.8889 \\
Algebraic geometry & 9 & 0.8889 \\
Thermodynamics & 8 & 0.8750 \\
Coordinate systems & 8 & 1.0000 \\
Numerical analysis & 8 & 1.0000 \\
Quantum mechanics & 8 & 0.8750 \\
Group theory & 8 & 0.8750 \\
Fluid dynamics & 7 & 0.8571 \\
Financial economics & 7 & 0.8571 \\
\hline
\end{tabular}
\caption{Top namespace-defining clusters discovered by $K$-Means with $K=8250$ on
LSA-space with $k=500$.}
\label{tab:strong-kmeans-svd}
\end{table}



\begin{table}[h!]
\centering
\begin{subtable}{0.7\textwidth}
\centering
\begin{tabular}{|c|c|}
  \hline
  Article & Identifiers \\
  \hline
Skew-symmetric matrix &  $\Sigma_a,\lambda_1,\theta,\lambda_2,\pi,B,\lambda_r,...$ \\
Diagonalizable matrix & $v_1,\lambda_1,v_k,\lambda_3,\lambda_2,\lambda_i,\lambda_k,\lambda_j,\lambda_n,...$ \\
Eigenvalues and eigenvectors & $v_i,\mu_A,\lambda_i,d,\lambda_n,...$ \\
Principal axis theorem & $v_1,u_1,\lambda_1,\lambda_2,D,S,u,...$ \\
Generalized eigenvector & $m,V,\lambda,\lambda_2,\lambda_1,\beta,k,...$ \\
Linear independence &  $\Lambda,v_j,u_2,v_3,u_n,\lambda_1,\lambda_3,\lambda_2,...$ \\
Symmetric matrix &  $\Lambda,\lambda_1,\lambda_2,D,Q,P,\lambda_i,...$ \\
\hline
\end{tabular}
\caption{Articles in the cluster ``Linear Algebra''.}
\label{tab:soft-kmeans-la}
\end{subtable}% mask EOL
\begin{subtable}{0.3\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
ID & Definition & Score\\
\hline
$D$ & diagonal matrix & 1.81 \\
$V$ & vector space & 5.26 \\
$t$ & real argument & 0.99 \\
$u$ & eigenvalues & 0.89 \\
$\Lambda$ & nonzero vector & 0.99 \\
$\theta$ & integer multiple & 0.83 \\
$\lambda$ & eigenvalue & 3.51 \\
$\lambda_1$ & eigenvalues & 4.40 \\
$\lambda_2$ & eigenvalues & 2.60 \\
$\lambda_i$ & complex number & 0.89 \\
$\lambda_k$ & eigenvalues & 0.99 \\
\hline
\end{tabular}
\caption{Definitions in ``Linear Algebra''.}
\label{tab:soft-kmeans-la-def}
\end{subtable}
\caption{A ``Linear Algebra'' cluster found by $K$-Means with $K=8250$ and $k=500$.}
\label{tab:strong-kmeans-lsa}
\end{table}


\begin{table}
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  \multicolumn{4}{|c|}{$\lambda$}\\
  \hline
  Size & Namespace Name & Definition & Score \\
  \hline
5 & Analytic geometry & odd multiple & 0.89 \\
4 & Analytic number theory & modular lambda function & 1.88 \\
3 & Applied and interdisciplinary physics & wavelength & 3.57 \\
4 & Cartographic projections & longitude & 6.36 \\
5 & Cartography & longitude & 6.37 \\
5 & Chemical kinetics & rate & 0.83 \\
3 & Complex analysis & forces & 0.93 \\
8 & Coordinate systems & longitude & 7.99 \\
6 & Electromagnetic radiation & wavenumber & 1.86 \\
3 & Electromagnetic spectrum & wavelength & 0.99 \\
6 & Electronic amplifiers & typical value & 0.93 \\
5 & Electronic engineering & wavelength & 0.89 \\
7 & Fluid dynamics & wavelength & 4.63 \\
6 & Group theory & limit ordinal & 0.97 \\
3 & Infinity & limit ordinals & 2.68 \\
4 & Lagrangian mechanics & lagrange & 0.89 \\
3 & Large numbers & ordinals & 1.80 \\
7 & Linear algebra & eigenvalue & 3.51 \\
4 & Materials science & wavelength & 0.89 \\
5 & Mathematical analysis & shape & 1.78 \\
4 & Mathematical physics & measure & 0.86 \\
5 & Measure theory & lebesgue measure & 0.95 \\
6 & Mechanics & previous expression & 0.95 \\
3 & Multilinear algebra & natural isomorphisms & 0.84 \\
3 & Number theory & liouville function & 0.93 \\
6 & Operator theory & identity function & 0.86 \\
3 & Optics & wavelength & 1.70 \\
3 & Philosophy of physics & kinds & 0.81 \\
7 & Physical constants & wavelength & 0.89 \\
6 & Polarization & length & 1.85 \\
5 & Probability distributions & exponential distribution & 1.79 \\
4 & Probability distributions & shape parameter & 0.93 \\
3 & Probability theory & suitable choice & 0.83 \\
3 & Quantum field theory & coupling constant & 1.94 \\
3 & Quantum information science & state & 2.66 \\
4 & Quantum mechanics & wavelength & 0.99 \\
5 & Radio technology & wavelength & 2.80 \\
7 & Rubber properties & engineering strain & 8.96 \\
3 & Statistical theory & single number & 0.99 \\
3 & Statistics & rate & 1.97 \\
3 & Theoretical physics & eigenvalues & 1.91 \\
4 & Transforms & eigenvalues & 1.82 \\
3 & Wireless & wavelength & 1.90 \\
\hline
\end{tabular}
\caption{Some of definitions of ``$\lambda$'' in the clustering obtained with $K$-Means.}
\label{tab:strong-kmeans-lambda}
\end{table}


Like for the weak association case, let us consider a cluster with documents on
Linear Algebra  (see table~\ref{tab:soft-kmeans-la}). We can observe that it
overlaps with the Linear Algebra discovered previously: there are also
``Diagonalizable matrix'', ``Eigenvalues and eigenvectors''
``Principal axis theorem'', ``Linear independence'' and ``Symmetric matrix''
articles. The extracted definitions are also similar (see table~\ref{tab:soft-kmeans-la-def}).
Let us also consider all definitions of ``$\lambda$'' across all namespaces:
there are 69 occurrences of ``$\lambda$'' (see table~\ref{tab:strong-kmeans-lambda}).

We do not attempt to perform Non-Negative Matrix Factorization as we have previously
established that it usually does not give better results while taking significantly
longer time.


\subsubsection{Russian Wikipedia} \ \\

Based on the experiments we have performed on English Wikipedia, we see that the best
performance is obtained with weak association by using MiniBatch $K$-Means on
LSA space reduced by SVD.
In this section we apply the best performing technique on Russian Wikipedia.

The identifier-document matrix has the dimensionality of $3948 \times 5319$
with 79171 non-zero elements, so the density of this matrix is 0.0038.


\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{k-vs-kmeans-rus.pdf}
\caption{Performace of $K$-Means with SVD for Russian Wikipedia.}
\label{fig:k-vs-kmeans-rus.pdf}
\end{figure}

As usually, we applied SVD with different values of rank $k \in \{150, 250, 350\}$,
and, similarity to no-definitions case for English Wikipedia, we do not
observe significant differences across different values of $k$
(see fig.~\ref{fig:k-vs-kmeans-rus.pdf}).
The best results with 105 namespace-defining clusters and with overall purity of 0.73 is
obtained by $K=3000$ and $k = 250$, and the largest namespace-defining clusters
are shown in table~\ref{tab:rus-wiki-categories}. Interestingly, there is a cluster
``Животные'' (``Animals'') where mathematical formulae are used to describe ``tooth formula''.
Let us consider a cluster about Linear Algebra (see table~\ref{tab:rus-la})
and definitions extracted from it (see table~\ref{tab:rus-la}). Similarity to English wikipedia,
some of the definitions are correct and valid, for example, ``сингулярный число''
(``singular value'') for ``$\sigma$''  or ``ранг'' (``rank'') for ``$r$'', while some
are not quite correct, e.g. ``скаляр'' (``scalar'') for ``$\lambda$''.
Additionally, some of the non-valid definitions seem to result from misclassifications
by the POS-tagger, for example, ``$\Sigma$'' is defined as ``вдоль'' (literally ``along''),
which do not make much sense.
Additionally we can look at all definitions of ``$\lambda$'' across all discovered namespaces
(see table~\ref{tab:rus-lambda}).

\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  Article (Original name) & Article (English) & Size & Purity \\
  \hline
Общая алгебра & Algebra & 7 & 0.8571 \\
Диф. геометрия и топология & Differential geometry and topology & 7 & 1.0000 \\
Диф. геометрия и топология & Differential geometry and topology & 6 & 0.8333 \\
Функциональный анализ &  Functional analysis & 6 & 0.8333 \\
Животные & Animals & 6 & 0.8333 \\
Картография & Cartography & 6 & 1.0000 \\
Математический анализ & Mathematical analysis & 5 & 1.0000 \\
Математический анализ & Mathematical analysis & 5 & 0.8000 \\
Теория вероятностей & Probability theory & 5 & 1.0000 \\
Механика & Mechanics & 5 & 0.8000 \\
Диф. уравнения в частных производных & Partial differential equations & 5 & 0.8000 \\
Математический анализ & Mathematical analysis & 5 & 0.8000 \\
Релятивистские и гравитационные явления & Relativity and gravitation & 5 & 0.8000 \\
Линейная алгебра & Linear algebra & 5 & 1.0000 \\
Математический анализ & Mathematical analysis & 5 & 1.0000 \\
Физика твёрдого тела & Solid-state physics & 5 & 0.8000 \\
\hline
\end{tabular}
\caption{Largest namespace-defining clusters extracted from Russian Wikipedia.}
\label{tab:rus-wiki-categories}
\end{table}

\begin{table}[h!]
\centering
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c|c|c|}
  \hline
  Article (Original name) & Article (English) & Identifiers \\
  \hline
Линейная алгебра & Linear algebra &  $V, v_n, \alpha, v_1, v_2, x, \alpha_1, \beta, \lambda, f, U,...$ \\
Спектральная теорема & Spectral theorem & $\Lambda, \lambda, H, K, P, U, T, V, X, f, y, x,...$ \\
Сингулярное разложение & Singular value decomposition & $\Sigma, V_k, \sigma, M, U, T, V, k, r, u, v,...$ \\
\begin{tabular}[x]{@{}c@{}} Ковариантность и \\ контравариантность \end{tabular}
 & Covariance and contra-variance & $S, V, d, g, f, k, m, f_i, n, u, v, x,...$ \\
Теорема Куранта -- Фишера & Courant–Fischer theorem & $k, V, S, L_k,...$ \\
\hline
\end{tabular}
\caption{A namespace-defining cluster about Linear algebra.}
\label{tab:rus-la}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c|c|c|c|}
  \hline
  ID & Definition & Definition (English) & Score \\
  \hline
$H$ & гильбертов & hilbert & 0.95 \\
$L$ & отображение & transformation & 3.69 \\
$L_k$ & оператор & operator & 0.87 \\
$M$ & воздействие матрица & matrix & 1.77 \\
$T$ & линейный отображение & linear transformation & 0.93 \\
$U$ & унитарный матрица & unitary matrix & 1.77 \\
$V$ & пространство & space  & 5.57 \\
$g$ & билинейный форма & bilinear form & 1.78 \\
$r$ & ранг & rank & 0.99 \\
$x$ & собственный вектор & eigenvector & 0.95 \\
$\Lambda$ & диагональный матрица & diagonal matrix & 2.76 \\
$\Sigma$ & вдоль & ``along'' & 0.94 \\
$\lambda$ & скаляр & scalar & 0.99 \\
$\sigma$ & сингулярный число & singular value & 0.96 \\
\hline
\end{tabular}
\caption{Definitions in the ``Linear Algebra'' namespace.}
\label{tab:rus-la-def}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  \multicolumn{6}{|c|}{$\lambda$}\\
  \hline
  Size & Original name & English name & Original definition & English definition & Score \\
  \hline
3 & Алгебра & Algebra & поль & field & 1.90 \\
5 & Гидродинамика & Fluid dynamics & тепловой движение & thermal motion & 0.89 \\
4 & Гравитация & Gravitation & коэф. затухание & damping coefficient & 0.99 \\
6 & Картография & Cartography & долгота & longitude & 4.75 \\
5 & Линейная алгебра & Linear algebra & скаляр & scalar & 0.99 \\
4 & Оптика & Optics & длина & length & 2.75 \\
3 & Оптика & Optics & длина волна & wavelength & 0.95 \\
5 & \begin{tabular}[x]{@{}c@{}} Релятивистские и \\ гравитационные явления \end{tabular} & \begin{tabular}[x]{@{}c@{}} Relativity and \\ gravitation \end{tabular} & частота & frequency & 0.89 \\
3 & Статистическая физика & Statistical physics & итоговый выражение & final expression & 0.89 \\
3 & \begin{tabular}[x]{@{}c@{}} Теоремы \\ комплексного анализа \end{tabular}  & \begin{tabular}[x]{@{}c@{}} Theorems of \\ complex analysis \end{tabular}  & нуль порядок & ``zero order'' & 0.96 \\
3 & Теория алгоритмов & Algorithms & функция переход & transition function & 2.86 \\
5 & Физические науки & Physical sciences & длина & length & 0.93 \\
  \hline
\end{tabular}
\caption{Definitions of ``$\lambda$'' across all namespaces.}
\label{tab:rus-lambda}
\end{subtable}
\caption{Namespaces extracted from Russian wikipedia.}
\label{tab:rus-namespaces}
\end{table}


\subsection{Building Hierarchy} \label{sec:hierarchy}


After the namespaces are found, we need to organize them into a hierarchical
structure. It is hard to do automatically, and we choose to use
existing hierarchies for mathematical knowledge, and then map the
found namespaces to these hierarchies.

The first hierarchy that we use is ``Mathematics Subject Classification'' (MSC)
hierarchy \cite{ams2010msc} by the American Mathematical Society, and it
is used for categorizing mathematical articles. In this scheme there are
64 top-level categories such as ``Mathematical logic'', ``Number theory'',
or ``Fourier analysis''. It also includes some physics categories such
as ``Fluid mechanics'' or ``Quantum Theory''. The following top level
categories are excluded: ``General'', ``History and biography'' and
``Mathematics education''.

Each top-level category contains second-level categories and third-level
categories. In this work we exclude all subcategories those code
ends with 99: they are usually ``Miscellaneous topics'' or
``None of the above, but in this section''.

Additionally, we excluded the following second level categories because
they interfere with PACS, a hierarchy for Physics:

\begin{itemize}
\item Quantum theory $\to$ Axiomatics, foundations, philosophy
\item Quantum theory $\to$ Applications to specific physical systems
\item Quantum theory $\to$ Groups and algebras in quantum theory
\item Partial differential equations $\to$ Equations of mathematical physics and other areas of application
\end{itemize}


% \begin{itemize}
% \item Statistics $\to$ Sufficiency and information
% \item Functional analysis $\to$ Other (nonclassical) types of functional analysis
% \item Functional analysis $\to$ Miscellaneous applications of functional analysis
%\end{itemize}

The second hierarchy is ``Physics and Astronomy Classification Scheme'' (PACS)
\cite{aps2010pacs}, which is a scheme for categorizing articles about Physics.
Like in MSC, we remove the top-level category  ``GENERAL''.

Finally, we also use the ACM Classification Scheme \cite{rous2012acm}
available as a SKOS \cite{miles2005skos} ontology at their website \cite{amc2012ccs}.
The SKOS ontology graph was processed with RDFLib \cite{rdflib}.
We use the following top level categories:
``Hardware'', ``Computer systems organization'', ``Networks'',
``Software and its engineering'', ``Theory of computation'',
``Information systems'', ``Security and privacy'',
``Human-centered computing'', ``Computing methodologies''.

After obtaining and processing the data, the three hierarchies
are merged into one.


However these categories are only good for English articles and
a different hierarchy is needed for Russian. One of such hierarchies is
``Госу\-дар\-ствен\-ный руб\-ри\-ка\-тор научно-тех\-ни\-чес\-кой инфор\-ма\-ции''
(ГРНТИ)~-- ``State categorizator of scientific and technical information'', which
is a state-recommended scheme for categorizing scientific articles published
in Russian  \cite{feodosimov2000grnti}. The hierarchy  is extracted from the
official website\footnote{\url{http://grnti.ru/}}. It provides
a very general categorization and therefore we keep only the following math-related
categories: ``Астрономия'' (``Astronomy''), ``Биология'' (``Biology''),
``Информатика'' (``Informatics''), ``Математика'' (``Mathematics''),
``Механика'' (``Mechanics''), ``Ста\-тис\-тика'' (``Statistics''),
``Физика'' (``Physics''), ``Химия'' (``Chemistry''),
``Экономика. Экономические Науки'' (``Economics'') and others.


One we a hierarchy is established, each found namespace is mapped to
the most suitable second-level category. This is done by keywords matching.
First, we extract all key words from the category, which includes
top level category name, subcategory name and all third level categories.
Then we also extract the category information from the namespace, but
we also use the names of the articles that form the namespace.
Finally, the keyword matching is done by using the cosine similarity
between the cluster and each category. The namespace is assigned to the
category with the best (largest) cosine score.

If the cosine score is low (below $0.2$) or there is only one
keyword matched, then the cluster is assigned to the ``OTHERS''
category.

For example, consider a namespace  derived from the cluster consisting of
``Tautology (logic)'', ``List of logic systems'', ``Regular modal logic''
``Combinational logic'' documents. Among others, these articles belong to categories
``Mathematical logic'' and ``Logic''. Then the following is the list of keywords
extracted from the cluster:
``tautology'', ``logic'', ``list'', ``systems'', ``regular'', ``modal'', ``combinational'',
``logical'', ``expressions'', ``formal'', ``propositional'', ``calculus'' and so on.
Apparently, this namespace is about mathematical logic.

Then consider a list of keywords for ``'General logic'', a subcategory of
``Mathematical logic and foundations'' from MSC:
``mathematical'', ``logic'', ``foundations'', ``general'', ``classical'', ``propositional'', ``type'', ``subsystems'' and others.

These keywords are represented as vectors in a vector space and the cosine score
between these vectors is calculated. For this example, the cosine is
approximately 0.75, and this is the largest similarity, and therefore this namespace
is mapped to the ``General logic'' subcategory.

Unfortunately the mapping is not always correct.


For example, let us consider ... the best clustering with 400+ discovered namespaces
from LSA with SVD and $K$-Means.

The majority of namespaces are mapped correctly. For example:

\begin{small}
\begin{itemize}
  \item ATOMIC AND MOLECULAR PHYSICS
    \begin{itemize}
      \item Atomic properties and interactions with photons (wiki: Atomic physics; Quantum mechanics; Atomic, molecular, and optical physics)
    \end{itemize}

  \item Algebraic geometry
    \begin{itemize}
      \item Computational aspects in algebraic geometry (wiki: Sheaf theory, Theorems in geometry, Theorems in algebraic geometry
      \item Computational aspects in algebraic geometry (wiki: Algebraic geometry, Algebraic varieties, Manifolds)
      \item Surfaces and higher-dimensional varieties (wiki: Algebraic varieties, Threefolds, Surfaces
    \end{itemize}

  \item Algebraic topology
    \begin{itemize}
      \item Fiber spaces and bundles (wiki: Differential geometry, Fiber bundles, Topology)
      \item Spectral sequences (wiki: Abstract algebra, Homological algebra, Algebraic topology)
      \item Applied homological algebra and category theory (wiki: Continuous mappings, Algebraic topology, Homotopy theory)
    \end{itemize}

  \item Biology and other natural sciences
    \begin{itemize}
      \item Mathematical biology in general (wiki: Evidence-based practices, Public health, Epidemiology)
      \item Genetics and population dynamics (wiki: Population genetics, Genetics, Subfields and areas of study related to evolutionary biology)
    \end{itemize}

  \item  Computing methodologies
    \begin{itemize}
      \item Machine learning (wiki: Machine learning, Learning, Artificial intelligence)
      \item Machine learning (wiki: Statistical data types, Multivariate statistics, Statistical classification)
    \end{itemize}

  \item Information systems
    \begin{itemize}
      \item Data management systems (wiki: Databases, Information technology management, Computer data)
    \end{itemize}
\end{itemize}
\end{small}


Some are somewhat accurate:

\begin{small}
\begin{itemize}
  \item Computer systems organization
    \begin{itemize}
      \item Real-time systems (wiki: Computer languages, Type systems, Data types;
            matched keywords: languages computer systems architecture)
    \end{itemize}

\item  Fluid mechanics
    \begin{itemize}
      \item Biological fluid mechanics (wiki: Fluid mechanics, Soft matter, Gases;
             matched keywords: mechanics fluid)
      \item Biological fluid mechanics
             (wiki: Fluid dynamics, Fluid mechanics, Computational fluid dynamics;
             matched keywords: mechanics fluid)
    \end{itemize}
\item Functional analysis
    \begin{itemize}
      \item Distributions, generalized functions, distribution spaces
             (wiki: Probability distributions, Exponential family distributions, Continuous distributions;
             matched keywords: analytic distribution distributions generalized)
    \end{itemize}
\item $K$-theory
    \begin{itemize}
      \item Whitehead groups and $K_1$
             (wiki: Group theory, Subgroup properties, Metric geometry;
             matched keywords: group subgroup)
    \end{itemize}

\item Partial differential equations
    \begin{itemize}
      \item Close-to-elliptic equations (wiki: Differential equations, Numerical analysis, Numerical differential equations;
             matched keywords: partial differential equations)
    \end{itemize}
\end{itemize}
\end{small}


Finally, namespaces marked as ``OTHER'' are usually matched incorrectly:

\begin{small}
\begin{itemize}
  \item OTHER
    \begin{itemize}
   \item Randomness, geometry and discrete structures
             (wiki: Coordinate systems, Cartography, Cartographic projections;
             matched keywords: projections)
   \item Other generalizations
             (wiki: Electrostatics, Concepts in physics, Electromagnetism;
             matched keywords: potential)
   \item Computational methods
             (wiki: General relativity, Exact solutions in general relativity, Equations;
             matched keywords: relativity)
   \item Other classes of algebras
             (wiki: International sailing classes, Keelboats, Olympic sailboat classes;
             matched keywords: classes)
  \end{itemize}
\end{itemize}
\end{small}

\textbf{TODO: Here goes the Russian hierarchy}



\subsection{Java Language Processing} \label{sec:jlp}

Previously we have illustrated the idea of identifier namespaces by comparing
it with namespaces in Computer Science, and it allowed us to develop an intuition
behind the namespaces in mathematics and also propose a method to discover them:
we motivated the assumption that there exist ``namespace defining''
groups of documents by arguing that these groups also exist in
programming languages.
In this section we will try to do the reserve: apply the methods
developed for identifier namespace discovery to the source code.

If a programming language is statically typed, like Java or Pascal,
usually it is possible to know the type of a variable from the declaration
of this variable. Therefore we can see variable names as ``identifiers''
and variable types as ``definitions''. Clearly, there is a difference
between variable types and identifier definitions, but we believe
that this comparison is valid because the type carries additional semantic
information about the variable and in what context it can be used --
like the definition of an identifier.

The information about variables and their types can be extracted from a
source code repository, and each source file can be processed to
obtain its Abstract Syntax Tree (AST). By processing the ASTs,
we can extract the variable declaration information. Thus, each
source file can be seen as a document, which is represented
by all its variable declarations.

In this work we process Java source code, and for parsing it
and building ASTs we use a library JavaParser \cite{javaparser}.
The Java programming language was chosen because it requires the programmer
to always specify the type information when declaring a variable.
It is different for other languages when the type information is
usually inferred by the compilers at compilation time.


In Java a variable can be declared in three places:
as an inner class variable (or a ``field''), as a method (constructor)
parameter or as a local variable inside a method or a constructor.
We need to process all three types of variable declarations
and then apply additional preprocessing, such as converting the name
of the type from short to fully qualified using the information from the
import statements. For example, \verb|String| is converted to
\verb|java.lang.String| and \verb|List<Integer>| to \verb|java.util.List<Integer>|,
but primitive types like \verb|byte| or \verb|int| are left unchanged.


Consider an example in the listing~\ref{code:javaclass}. There is a
class variable \texttt{threshold}, a method parameter \texttt{in} and
two local variables \texttt{word} and \texttt{posTag}. The following
relations will be extracted from this class: (``threshold'', \verb|double|),
(``in'', \verb|domain.Word|), (``word'', \verb|java.lang.String|),
(``posTag'', \verb|java.lang.String|).
Since all primitives and classes from packages that start with
\verb|java| are discarded, at the end the class \verb|WordProcesser|
is represented with only one relation (``in'', \verb|domain.Word|).


\begin{lstlisting}[language=Java,caption={A Java class},label={code:javaclass}]
package process;

import domain.Word;

public class WordProcesser  {

    private double threshold;

    public boolean isGood(Word in) {
        String word = in.getWord();
        String posTag = in.getPosTag();
        return isWordGood(word) && isPosTagGood(posTag);
    }

    // ...

}
\end{lstlisting}


In the experiments we applied this source code analysis to
the source code of Apache Mahout 0.10 \cite{mahout}, which is an open-source
library for scalable Machine Learning and Data Mining.
As on \today, this dataset consists of 1\,560 java classes with 45\,878
variable declarations. After discarding declarations from the standard Java API,
primitives and types with generic parameters, only 15\,869 declarations were
retained.

The following is top-15 variable/type declarations extracted from the Mahout
source code:

\begin{itemize}
\item ``conf'', \verb|org.apache.hadoop.conf.Configuration| (491 times)
\item ``v'', \verb|org.apache.mahout.math.Vector| (224 times)
\item ``dataModel'', \verb|org.apache.mahout.cf.taste.model.DataModel| (207 times)
\item ``fs'', \verb|org.apache.hadoop.fs.FileSystem| (207 times)
\item ``log'', \verb|org.slf4j.Logger| (171 times)
\item ``output'', \verb|org.apache.hadoop.fs.Path| (152 times)
\item ``vector'', \verb|org.apache.mahout.math.Vector| (145 times)
\item ``x'', \verb|org.apache.mahout.math.Vector| (120 times)
\item ``path'', \verb|org.apache.hadoop.fs.Path| (113 times)
\item ``measure'', \verb|org.apache.mahout.common.distance.DistanceMeasure| (102 times)
\item ``input'', \verb|org.apache.hadoop.fs.Path| (101 times)
\item ``y'', \verb|org.apache.mahout.math.Vector| (87 times)
\item ``comp'', \verb|org.apache.mahout.math.function.IntComparator| (74 times)
\item ``job'', \verb|org.apache.hadoop.mapreduce.Job| (71 times)
\item ``m'', \verb|org.apache.mahout.math.Matrix| (70 times)
\end{itemize}

We used the ``soft'' association method to incorporate ``definition''
(i.e. types), and considering each source code file as a document,
we build an identifier-document matrix of dimensionality
$1436 \times 1560$. Only identifiers that occur at least twice are used
to build the matrix.

Previously the best performance was achieved by using LSA and MiniBatch $K$-Means,
and therefore we apply the same algorithms here. However there are a lot of instances
of the types \texttt{Vector} and \texttt{Matrix}, and to mediate its influence, we use two variants of TF-IDF:
with usual TF component and with sublinear TF.
The best performance is achieved with the rank $k=200$ of SVD and
number of clusters $K=200$ using sublinear weighting (see fig.~\ref{fig:jlp-perf}).
% each experiment was repeated 10 times and we record the average


\begin{figure}[h!]
\centering
\hfill
\begin{subfigure}[b]{0.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{jlp-lens.pdf}
  \caption{Usual TF $\times$ IDF weighting}
  \label{fig:jlp-perf-tf}
\end{subfigure}
~
\begin{subfigure}[b]{0.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{jlp-lens-sublin.pdf}
  \caption{$(\log \text{TF}) \times \text{IDF}$ weighting}
  \label{fig:jlp-perf-subtf}
\end{subfigure}
\caption{The performance MiniBatch $K$-Means on the Mahout dataset.}
\label{fig:jlp-perf}
\end{figure}


With these parameters the best result is 33 clusters.
One of such clusters is a cluster about SVD: there are 5 classes
from the \verb|recommender.svd|\footnote{full name: \texttt{org.apache.mahout.cf.taste.impl.recommender.svd}} package
(\texttt{Factorization}, \texttt{FilePersistenceStrategy}, \texttt{NoPersistenceStrategy}, \texttt{PersistenceStrategy}, \texttt{FilePersistenceStrategyTest})
and one from \\ \verb|kddcup.track1.svd|\footnote{full name: \texttt{org.apache.mahout.cf.taste.example.kddcup.track1.svd}} package
(\texttt{Track1SVDRunner}).
Although this cluster is not 100\% pure, in the sense that not all of
these classes belong to the same package, these classes are
clearly related: they are all about SVD.
The top dimensions with the most influence in this cluster are
\verb|svd.Factorization|\footnote{full name: \texttt{org.apache.mahout.cf.taste.impl.recommender.svd.Factorization}}
and \texttt{factorization}.

% One of these
% clusters is \verb|org.apache.mahout.math.neighborhood| cluster with
% BruteSearch, FastProjectionSearch, LocalitySensitiveHashSearch, ProjectionSearch,
% Searcher, LocalitySensitiveHashSearchTest, SearchSanityTest. All these classes are
%related. Not all classes from this package are included. For example,
% HashedVector and LumpyData are not, and, judging by the name of these
%classes, they appear a bit different from the rest. Therefore
%these classes are indeed semantically related.
% There are many identifiers in this namespace


Note that there is a difference between mathematical namespaces and
namespaces discovered in the source code. The found ``namespaces'' do not necessarily
correspond to the real packages in the source code. The reason for this is
the document-centric view on the namespaces: for documents we assume that the
namespaces are not directly observed, and instead we can see only the documents where
these namespaces are used. It is not the case for real namespaces
in software: we do observe namespaces directly, and documents (that is, classes)
are also the elements of the namespaces.



\subsection{Result Analysis and Experiment Conclusions}


Hierarcical methods are too slow, and SLINK is not good.
%Bisecting $K$-Means is good for explaining steps but not very practical

MiniBatch K means is preferred to usual KMeans:
fast but same results

The baseline of random cluster assignment is beaten.

NMF takes a lot of time to decompose a matrix with large
$k$



The best definition embedding technique is soft association.
The best clustering algorithm is $K$-Means with $K=9500$
on the semantic space produced by rank-reduced SVD with $k = 250$
with TF-IDF weight where TF is sublinear.






